Joint Traffic Offloading and Aging Control in 5G IoT Networks

The widespread adoption of 5G cellular technology will evolve as one of the major drivers for the growth of IoT-based applications. In this paper, we consider a Service Provider (SP) that launches a smart city service based on IoT data readings: in order to serve IoT data collected across different locations, the SP dynamically negotiates and rescales bandwidth and service functions. 5G network slicing functions are key to lease an appropriate amount of resources over heterogeneous access technologies and different site types. Also, different infrastructure providers will charge slicing service depending on specific access technology supported across sites and IoT data collection patterns. We introduce a pricing mechanism based on Age of Information (AoI) to reduce the cost of SPs. It provides incentives for devices to smooth traffic by shifting part of the traffic load from highly congested and more expensive locations to lesser charged ones, while meeting QoS requirements of the IoT service. The proposed optimal pricing scheme comprises a two-stage decision process, where the SP determines the pricing of each location and devices schedule uploads of collected data based on the optimal uploading policy. Simulations show that the SP attains consistent cost reductions tuning the trade-off between slicing costs and the AoI of uploaded IoT data.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> bak/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> bak/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> sections/intro.tex <==
\section{Introduction}
%----------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Data collection at scale represents the key signature of future IoT applications, posing significant challenges in the integration of emerging 5G networks and IoT technologies as identified in early studies \cite{surveyIoT}. In fact, pervasive object readings  play a decisive role in the context of smart cities for both process monitoring and management. Using IoT, a whole new set of applications will be able to feed local information generated by both objects and mobile devices into their databases.

In IoT networks, local data streams are collected from heterogeneous information sources. Examples of sources include meters for water and electricity management, outdoor and indoor positioning data, parking presence sensors and a whole new set of user-generated contents related to application-specific data. Such information streams are consumed for management and prediction purpose by services such as  city air management, smart waste management or traffic management and demand-response schemes~\cite{zanella2014}.   

% Indeed, traditional utility service providers have long performed IoT data collection to reduce operational costs. Such traditional schemes are typically based on M2M to match the requirements of proprietary SCADA systems and charged per sms. As such, they appear inadequate in the context of emerging IoT systems. 


The long standing problem of integrated architectures and protocols to support IoT data collection appears now solved by the uptake of 5G connectivity \cite{cisco2020}. % whose second major driver, beyond multimedia traffic, is the current growth of mobile IoT connections.
%Actually, with both new LTE-M radio interface and the new suite of architectural paradigms, 5G introduces key infrastructural assets able to ease both IoT access to radio resources and computing at the edge of the network.  While such technological enablers will be key to cope with the scale of IoT data collection processes, 
In particular, slicing techniques offered by 5G technology allow Infrastructure Providers (InP) to offer differentiated services to their customers using shared resource pools. A slice, in this context, is a share of mobile network infrastructure obtained by forming a logical network on top of the physical one. %\emph{Hence, the 5G technology enables traffic offloading through slicing, i.e., nodes can dynamically offload traffic  from a given slice by switching across alternative slices. }
Traffic differentiation in 5G systems can be obtained by isolating specific traffic categories within slices, which in turn can be dedicated to serving target verticals under specific service isolation guarantees \cite{ZhangCommMag}\cite{SamdanisMT}. For this reason, slicing is deemed a key enabler for several strategic service domains, and are henceforth referred to as \emph{slicing services}. One premier class is that of smart city services, where Service Providers (SP) will be able to support IoT data readings from mobile sensing devices. In this context, the role of the SP is to lease resources (radio, processing, storage and  radio resources) in the form of one or more dedicated slices and from one or multiple InPs. 

A slice will support the connectivity of the fleet of devices taking part to the IoT sensing services at a cost for the upload of sensed data. 
%New Service Providers (SP) will launch smart city  services to support IoT data readings: such services represent one of the strategic vertical domains for the application of slicing in 5G networks \cite{zanella2014}, and are henceforth referred to as SP \emph{slicing services}. The SP leases resources (radio, processing, storage and  radio resources) from one or multiple InPs to  which the fleet of devices taking part to the IoT \emph{sensing service} will connect, at a cost,  in order to upload their sensed data.  
 However, the costs incurred by sensing services depend on a number of factors, including the business model and the ownership of the sensing devices. It is possible for instance that sensing devices are owned by the SP whereas the sensing services are designed and run by third parties and offered, e.g.,  as a smartphone app. In this case the sensing services involve payments to the SP~\cite{jayasumana2007virtual}. If the SP is in charge of the sensing services and also the slicing services%, in turn, it may still be the case that the two are run by separate divisions inside the SP, again involving financial costs among them. However, non-monetary costs -- in the form of shadow prices \cite{Kelly1998} -- can be used effectively as a penalty to avoid hot-spot phenomena by deterring the upload of sensed data in congested areas. 
in turn, non-monetary costs --  similar to the shadow prices defined in \cite{Kelly1998} -- can be used effectively as a penalty to avoid hot-spot phenomena by deterring the upload of sensed data in congested areas. 

In turn, IoT sensing services relying on 5G technology pose their own challenges. The informative content of sensed data changes over time depending on the profile of the IoT sensing service. Information on traffic mobility, for instance, will retain its value on the timescale of the tenths of seconds, whereas temperature and pollution measurements will change in the timescale of the hours. % For example, IoT is already one of the key sources for real-time data for Machine Learning (ML), and enables the decision of ML to be carried out. 
Clearly, IoT devices require a mechanism to control information freshness, the latter being also referred to as the \emph{age of information} (AoI).  Such mechanism, known as aging control, determines when IoT readings should be uploaded in order to avoid stale information. 
\begin{table}[t]\caption{Table of notation}
\centering
\begin{tabular}{p{0.3\columnwidth}|p{0.6\columnwidth}}
\hline
{\it Variable} & {\it Description}\\
\hline
${\Loc}=\{1,\ldots,L\}$ & set of regional locations\\
$\mathcal P=\{p_1,\ldots,p_K\}$  & set of upload unit prices\\
$\mathcal M=\{1,\ldots,M\}$  & set of information age values\\
$\Pi_{ij}$& transition probability from location $i$ to  $j$ \\
$\pi_{i}$& occupation probability of location $i$ \\
$a_{t}$& action at time $t$ \\
$s_{t}=(x_t,l_t)$& state at time $t$ \\
$x_t$& age of information at time $t$  \\
$l_t$& location at time $t$ \\
\hline
\end{tabular}\label{tab:notation}
\end{table}

Controlling the AoI dynamics of data carried by IoT devices permits to trade-off between the value of IoT sensing readings -- indeed specific to a tagged service -- for the cost for uploading them using the 5G IoT slicing service. Motivated by the aging control problem intrinsic to IoT devices, and by the traffic offloading capabilities enabled by 5G technology, in this paper we investigate the following two questions: 
\begin{enumerate}
\item given the requirements of a tagged \emph{IoT sensing service} and the SP charging rates, what is the optimal upload strategy to control information freshness at the device level? 
\item how should the SP charge users to incentivize them to offload IoT data in order to reduce the costs of the \emph{SP slicing service}?
\end{enumerate}
In this paper, we control the AoI in order to derive the optimal upload strategy for the IoT service provider. Sensing devices will trigger the upload of sensed data depending on two factors: the application profile and the price available for the IoT sensing service. The application profile determines for how long sensed data will maintain their value, whereas location-dependent prices will determine the unit cost of sensed data uploads performed on the IoT slices. We thus formulate the problem as a Markov decision process (MDP), and provide the structure of the optimal solution based on the average cost model. 
The optimal stationary policy solving the problem results of the multi-threshold type: the upload of information will occur depending on the upload prices available to a tagged device, i.e., prices available in the cell it is connected to, and on the AoI relative to the data stored in the device memory. 

{\em Prior art and main contribution. } The two control actions considered in this work are traffic offloading control and aging control. Traffic offloading is a standard networking technique which will be \emph{enabled} by 5G technology in a smooth way through slicing. Aging control is \emph{required} by sensing applications, as typical of IoT systems. Although there is a vast literature on those two problems separately ~\cite{altman2019forever, liu2020joint, song2019age,Raja2020,Kortoci2019}, prior work have not considered the two problems at once. The contribution of this paper aims to connect these two research lines within same control framework.

The main contribution of this work is a scheme for the cost efficient brokerage of IoT data using 5G slicing. The proposed scheme encompasses several new features with respect to the related literature (at the best of the authors' knowledge). While IoT data offloading techniques  have been designed in the recent literature, e.g., in the context of vehicular networks \cite{Raja2020} or sensor networks \cite{Kortoci2019}, we tailor our solution  for 5G slicing; furthermore, the upload control of IoT data is optimized in a fully distributed and location-aware fashion. Second,  by means of a flexible 
 pricing control, we minimize the cost incurred by the SP in order to lease slice resources from InPs. Third, our scheme includes a notion of SLA rooted in the concept of AoI: as such, it is able to capture the latency requirements of IoT data readings, as agreed by the SP with her customers. 

{\em Structure of the paper. } The remainder of this work is organized as follows. First we introduce the considered system in Sec.~\ref{sec2}.  Then, we discuss the two main pillars of our work, namely, traffic offloading and aging control in Sec.~\ref{sec3} and  in Sec.~\ref{sec4}, respectively.  Section~\ref{sec5} bridges the two pillars in a unified framework. We report numerical results in Sec.~\ref{sec6} and we revise related works in Sec.~\ref{sec7}. A closing section ends the paper.




==> sections/shadow-main.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}~\label{sec5}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 
%\begin{figure}[t!]
%\includegraphics[width=0.5\textwidth]{Pictures/flowdiagrams}
%\caption{Joint aging control and offloading}
%\end{figure}
%
\subsection{Pricing as a tool for joint aging control and offloading }

We recall that the SP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the average size of the collected data.  

First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for SP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy 
is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Pricing through constrained optimization}
\subsection{Joint  Offloading and Aging Control}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec4}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec3}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control (JOAC)}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for SP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.

The  \JOAC problem is a constrained non-linear integer valued optimization problem defined over the set of multi-threshold policies. Finding 
a solution is made difficult because the structure of function $Y$ is not convex over the shadow price vectors ${\bf p}$. In what follows we propose an algorithm which utilizes  the structure of the devices' optimal strategy to solve the problem 

%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulated annealing for optimal pricing }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the \JOAC  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$.  Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$.  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation of \JOAC becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
%&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  L({\bf s})  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf s}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{{\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$

%Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.

Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem. The algorithm is driven by the rationale according to which a shadow price vector should permit to offload as much traffic as possible towards locations with smaller costs. In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimization problems \cite{pincus70,connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way. 
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 
The neighborhood structure is essential in order to specialize SA to our JOAC problem. Let define neighboor set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. The interpretation is that the AoI constraint \eqref{C2} is satisfied for at least one threshold vector, i.e.,  $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $. As it will be clear in the rest of the discussion, restricting to ${\mathcal N}_i$ will permit to restrict the information collected by cell $j$ to its neighboring locations only, i.e., $j\in{\mathcal N}_i$. 
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use the probability distribution Boltzmann-Gibbs, which is  constructed for our \JOAC by 
\begin{equation}\label{eq:BG}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is a normalization constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that is
$$
\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
In practice, the SA algorithm we propose in the following operates a uniform sampling of the neighbourhood, based on the Metropolis--Hastings (MH) algorithm. Thus, the acceptance-rejection policy gives raise to a specific kernel for a Markov chain, named $Q_T$, which represents the stochastic model which converges to the sequence of samples from the probability distribution $\pi_T({\bf s})$. The uniform sampling of the neighborood of each state is defined by the symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$:
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L \, (t_{max}-1) }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\label{tran}
\end{align}
If the temperature is fixed, the transition matrix of the resulting time-reversible Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$, writes as follows: 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  {\bf s}\not={\bf s}'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  {\bf s}\not={\bf s}'\\
q^*({\bf s}, {\bf s})  +\sum_{{\bf z}}q^*({\bf s}, {\bf z}) (1-\min\{1, \frac{\pi_T({\bf z})}{ \pi_T({\bf s})}\} ) &\textrm{ if }  {\bf s}={\bf s}'\\
\end{array}
\right.
\end{align}
Finally, the following statement, whose proof is reported in Appendix, ensures the convergence to the target stationary distribution \eqref{eq:BG}
\begin{lemma}
\label{lem1}
The Markov chain with the above transition has as stationary distribution $\pi_T({\bf s})$.  
\end{lemma}

The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the standard cooling schedule in the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{theorem}
\label{theom_conv}
If $T_n$ assumes the parametric form 
\begin{equation}
T_n =\frac{a}{log(n+1)}
\end{equation}
where $a= \frac{N F}{T} max_{j\in{\cal L}} C_j$, then 
\begin{equation}
\lim_{n\to \infty} \pi_{T_n}(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'\in S_{\epsilon, d} } L({\bf s}')\})=1
\label{conv}
\end{equation}
\end{theorem}
The above theorem shows that the Markov chain with matrice transition  $Q_{T_n}$,  converges to the constrained optimal threshold $s^*\in S^*$ with probability one when $n$ goes to $+\infty$, where $S^*$ is the set of the optimal solutions of the \JOAC problem.
\begin{proof}
Our proof for the theorem is based on the technique introduced in \cite{hajek88}, in which the annealing optimality of the original SA is proven.  
%We need only to show that $c$ is bigger than the maximum of the depths of  all state of the Markov chain.
Note that the objective function $L$ is nonnegative and the maximum positive value of $L$ is attained when data are collected by all devices at locations where the cost is maximal. Thus $a >  L({\bf s}')$ for all state $s$ and thus $a > d^*$, where $d^*$ is the maximum of the depth of all states which are local but  not global minima. We have 
\begin{eqnarray}\label{eq:suffcond}
\sum_{n=1}^{\infty} \exp^{-d^*/T_n}&=& \sum_{n=1}^{\infty} \exp^{(-\frac{d^*}{a} log(n+1))}\\
& >&  \sum_{n=1}^{\infty} \exp^{- log(n+1)} \\
&=& \sum_{n=1}^{\infty} \frac{1}{n+1} = +\infty 
\end{eqnarray}
Theorem 1 in \cite{hajek88} ensures the equivalence of \eqref{eq:suffcond} and \eqref{conv}, which completes the proof of Theorem \ref{theom_conv}.
\end{proof}

Hereafter, we describe the detailed implementation of the  simulated algorithm for solving the  \JOAC  problem. Time is divided into discrete slots where each time slot $t$ consists of three phases: selection, testing and decision. The pseudocode of the Algorithm is reported in Fig.~\ref{algo}. In line $1$, we initiate the threshold for all location to zero. This corresponds that all allocation adopt price $p=0$. Line $2$ initializes the temperature to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{\log(n)}$. In line $4$, the SP selects a location uniformly at random. Line $5$ describes how a new state is generated from a selected location. Line 6 indicates that the strategies of other location are  not changed.  Lines $7-11$ test if the new generated state ${\bf s}(t)$ is accepted or not. Line $12$  sets the condition to stop the SA algorithm. 

\begin{algorithm}[t]
 \caption{Simulated Annealing (SA) algorithm for \JOAC \label{algo}}
 \begin{small}
 \begin{algorithmic}[1]
 \STATE  Initialize:  $s_j(0)=0$, for all  $j\in{\cal L}$
 \STATE Set starting temperature $T_0= T^0$\\
 {\bf Selection  phase (in time slot n)}
\STATE Set temperature $T_n=\frac{c}{\log(n)}$
\STATE SP selects a location $i$  uniformly
\STATE Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly
\STATE Set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$\\
{\bf Test phase (at time slot n)}
\STATE  Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d))$; 
\STATE Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} 
\IF{the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$}
\STATE go to step 
\ELSE
\STATE go back to step $4$ (selection phase)
\ENDIF
\STATE Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$
\IF{$\delta < 0$}
\STATE $(s(t-1)$ is replaced by new state
\ELSE   
\STATE $s(t)=(s(t-1)$ with probability  $1-e^{\delta/T_n}$
\ENDIF\\
{\bf Stopping condition: }
\STATE the current configuration is not changed for two successive timeslots or $T_n <\varepsilon$
\end{algorithmic}
 \end{small}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Accelerated Simulated Annealing (SA) using  coloring approach}

To accelerate the algorithm, we can exploit the idea of independent sets of locations, i.e., a partition of locations into groups where locations within each group would not be affected by a change of threshold values that may occur in other locations of the same group. In practice, the speedup is obtained since the algorithm can be run in parallel for all the locations that belong to the same group. Our experiments demonstrate that this parallelization can attain a two-fold speedup of the run time with respect to the basic implementation of the algorithm. 

A partition into independent locations can be obtained as the result of a graph coloring procedure. The coloring of a graph is a function that assigns different colors to adjacent vertices of a graph. The Graph Coloring Problem seeks the minimum number of colors which can be used to color a graph. Such a number is called the chromatic number. An upper bound for the chromatic number is given by $\Delta + 1$ where $\Delta$ is the maximum degree of the graph and such bound is attained by the greedy coloring procedure. However, while optimal coloring is an $\mathcal {NP}$-hard problem, such upper bound may be loose for general graphs.

 %, up on coloring the entire graph, vertices that belong to a color does not contain an edge with any of the other vertices, which is exactly what is needed to update the thresholds of independent locations in parallel by assuming each location as a vertex and connecting its neighbous through an edge. 

Interestingly, Simulated Annealing can be used to solve this problem \cite{SAcoloring2} as well. We can thus incorporate the coloring process and the resulting parallelization into the algorithm shown in Fig.~\ref{algo} with a slight modification. The resulting implementation is reported in Fig ~\ref{intandom}.

The location coloring is obtained by using a specialized simulated annealing algorithm. Let $V= \lbrace v_1, v_2, v_3, \ldots v_L\rbrace$  be the set of colors that can be assigned to a location. We define a coloring $c: V \rightarrow \L$ a function assigning elements of $V$ to $\L$. A coloring is {\em feasible} if, for any pair of locations $i, j$ such that $i\in {\mathcal N}_j$, we have $c(j)\not = c(i)$, where $c(k)$ is the color of location $k$. Let $V({\bf c})$ be the set of colors used at state ${\bf c}=(c(1),c(2),..,c(L))$. Thus the objective of coloring problem  is to find a feasible solution that minimizes  the cardinality of set $V({\bf c})$, denoted by $E({\bf c})$. The algorithm begins with an initial feasible coloring scheme which is obtained by greedy algorithm then, improve it further using simulated annealing.

Now, we present the description of the algorithm depicted in Alg.~\ref{algo2}. In line $1$, the algorithm chooses a location and in line $2$, the chosen location selects randomly a color from $V\textbackslash\{c_{t-1}(i)\}$. Line $3$ indicates that the colors of other locations are not changed. Lines $4$-$14$ test if the new state is accepted or not. Lines $6$-$14$ test if the newly generated state ${\bf c}_t$ is accepted or not. Line $15$  indicates the output of algorithm  \ref{algo2} at each time step. 

Finally, the accelerated simulated annealing is obtained by integrating the coloring iteration into the main Algo.~\ref{algo} as shown in Fig.\ref{algo2}. At each time step, the SA algorithm for the optimal threshold search can be run in parallel at multiple locations overall locations with the same color (line $4$ in Algo.~\ref{algo}) only if the current output of the coloring algorithm is better than the previous output. As in the basic implementation, such locations generate a new threshold strategy and test if the new state is accepted or not (lines $6$-$19$ in Algo.~\ref{algo}).
 
\begin{algorithm}[t]
 %\caption{Pseudocode for the accelerated SA algorithm (in time slot $n$)\label{algo2}}
 \caption{Pseudocode for the SA-based coloring agorithm\label{algo2}}
 \begin{small}
 \begin{algorithmic}[1]
 \STATE  The network selects a location $i\in {\cal L}$.
 \STATE The  location $l$  chooses a color  $c \in V\textbackslash\{c_{t-1}(i)\}$ and set $c_t(i)= c$.
 \STATE Set $c_t(j) = c_{t-1}(j) \forall j \in {\mathcal L} \textbackslash \{l\}$ \\
 \IF{ the new state ${\bf c}_t$ is feasible}
     \STATE go to step 6 
     \ELSE 
     \STATE  go to step 3
 \ENDIF
\STATE  Set $\gamma  = E({\bf c}_t)-E({\bf c}_{t-1})$ 
\IF{ $\gamma$ < 0} 
\STATE the state ${\bf c}_{t-1}$ is replaced by new state   ${\bf c}_{t}$
\ELSE
\STATE  ${\bf c}_{t} = {\bf c}_{t-1}$ with probability  $1-e^{\gamma/\tilde T_n}$
\ENDIF
\STATE {\bf Output}   ${\bf c}_{t}$  and  $E({\bf c}_{t})$
\end{algorithmic}
 \end{small}
\end{algorithm}


\begin{figure}[h]
%\vspace{-1cm}
	\centering 
	\includegraphics[width=0.8\textwidth]{./pictures/flowchart2.pdf}
	\put(-300,200){\Large pippo}
	%\vspace{-2cm}
	\caption{The accelerated SA algorithm: at each step groups are generated using coloring}\label{intandom}
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
\end{figure}
 
 


   





==> sections/shadow5.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}~\label{sec5}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 
%\begin{figure}[t!]
%\includegraphics[width=0.5\textwidth]{Pictures/flowdiagrams}
%\caption{Joint aging control and offloading}
%\end{figure}
%
\subsection{Pricing as a tool for joint aging control and offloading }

We recall that the SP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the average size of the collected data.  

First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for SP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy 
is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Pricing through constrained optimization}
\subsection{Joint  Offloading and Aging Control}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec4}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec3}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control (JOAC)}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for SP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.

The  \JOAC problem is a constrained non-linear integer valued optimization problem defined over the set of multi-threshold policies. Finding 
a solution is made difficult because the structure of function $Y$ is not convex over the shadow price vectors ${\bf p}$. In what follows we propose an algorithm which utilizes  the structure of the devices' optimal strategy to solve the problem 

%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulated annealing for optimal pricing }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In the \JOAC  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$.  Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$.  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation of \JOAC becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
%&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  L({\bf s})  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf s}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{{\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$

%Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.

Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem. The algorithm is driven by the rationale according to which a shadow price vector should permit to offload as much traffic as possible towards locations with smaller costs. In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimization problems \cite{pincus70,connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way. 
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 

The neighborhood structure is essential in order to specialize SA to our JOAC problem. Let define neighboor set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. The interpretation is that the AoI constraint \eqref{C2} is satisfied for at least one threshold vector, i.e.,  $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $. As it will be clear in the rest of the discussion, restricting to ${\mathcal N}_i$ will permit to restrict the information collected by cell $j$ to its neighboring locations only, i.e., $j\in{\mathcal N}_i$. 
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use the probability distribution Boltzmann-Gibbs, which is  constructed for our \JOAC by 
\begin{equation}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is a normalization constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that is
$$
\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

We now  construct the transition of the Markov chain, named $Q_T$,  that can be used to obtaining a sequence of samples from the probability 
distribution $\pi_T({\bf s})$.  We start by defining a symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$ as follows
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L \, t_{max} }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
This is the matrix that correspond to the uniform sampling of the neighborood of each state ${\bf s},$ operated by the SA algorithm. The transition matrix of the Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$,  for a given temperature $T$, can be  constructed as follows: 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  {\bf s}\not={\bf s}'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  {\bf s}\not={\bf s}'\\
q^*({\bf s}, {\bf s})  +\sum_{{\bf z}}q^*({\bf s}, {\bf z}) (1-\min\{1, \frac{\pi_T({\bf z})}{ \pi_T({\bf s})}\} ) &\textrm{ if }  {\bf s}={\bf s}'\\
\end{array}
\right.
\label{tran}
\end{align}
\begin{lemma}
\label{lem1}
The Markov chain with the above transition has as stationary distribution $\{\pi_T({\bf s})\} $.  
\end{lemma}
\begin{proof}
See appendix C
\end{proof}
%It is shown in \cite{Hammaersly64} that a Markov chain with the above transition has as stationary distribution $\{\pi_T({\bf s})\} $.  
%\begin{table}
%\caption{Notation for SA algorithm}
%\begin{tabular}{ll}
%\hline
%Variable & Description \\
%\hline
%\hline
%$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
%$\mathcal{N}$ & physical  adjacency matrix \\
%$Q$ & infinitesimal generating matrix \\
%$T$ & temperature of SA algorithm \\
%$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
%${\pi}_i$ & steady state occupancy of cell $i$ \\ 
%$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
%$s$ & vector of thresholds \\
%\hline
%\end{tabular}
%\end{table}
%
The most distinctive feature of SA is it that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{T}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the standard cooling schedule, i.e., $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
The simulated annealing (SA) algorithm for the \JOAC problem.\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{log(n)}$\\
4: SP selects a location $i$  uniformly; \\
5: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly;\\
6: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$;  \\
{\bf Test phase (at time slot n)}\\ 
7: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
8:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
9: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  go back to step $3$ (selection phase);\\
10: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
11: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 12: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$)\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Simulated annealing}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Hereafter, we present how to implement the  simulated algorithm for solving the  \JOAC  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: selection, testing  and decision. The Algorithm reported in Fig.~\eqref{algo}  presents our global minimization algorithm.

In line $1$, we initiate the threshold for all location to zero. This corresponds that all allocation adopt price $p=0$. Line $2$ initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{\log(n)}$.   In line $4$, the SP selects a location uniformly at random. Line $5$ describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines $7-11$ test if the new generated state ${\bf s}(t)$ is accepted or not. Line $12$  sets the condition to stop the SA algorithm. 
%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution can be done similarly to that of \cite{Bremaud99} based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*\in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the \JOAC problem.
\end{theorem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulated annealing with coloring}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
One of the common drawbacks of the SA algorithm mentioned in the literature is longer run time, for this reason, we propose a method to improve the run time. This can be achieved by dividing cells into independent sets such that no set contains a cell and its neighbor and test all the cells in one such set per each temperature setting as opposed to testing one cell per each temperature setting. This is achieved by transforming the cell topology as a graph with cells as vertices, connecting each cell with its neighbors with an edge, and modeling it as \textsc{Graph Coloring Problem (GCP)}, a well-studied problem in graph theory.

The aim of this problem is to fully color the graph with a minimum number of colors, which is often referred to as \textit{chromatic number}. A large part of the literature is focused on coloring the graph given a number of colors \cite{coloring1}\cite{coloring2}, which doesn't address the problem of obtaining chromatic number or near-optimal minimum colors. \cite{Kirkpatrick671}\cite{SAcoloring1}\cite{SAcoloring2} address optimization by simulated annealing and \textsc{GCP} in greater detail. Obtaining the minimum number of colors is achieved using the SA algorithm, However, it is achieved rather in an indirect way. For this reason, we propose a simple and straight forward algorithm which is very similar in its structure to the SA algorithm described in the previous section. This algorithm is illustrated in fig.\ref{fig6}. Inspiration is drawn from \cite{SAcoloring2}, however the implementation is different from it. Let us consider a set of vertices drawn from the cell topology $ {\bf v} = \lbrace v_1, v_2, v_3, . . . v_N\rbrace$, set of colors used to color vertices are ${\bf c} = \lbrace c_1 , c_2, c_3, . . . c_K \rbrace$ and 
\begin{align*}
{\mathcal E_i} =
 \left\{
\begin{array}{ll}
1; \ if \ vertex \ i \ contains \ a \ bad \ edge \ with \\ \hspace{0.4cm}atleast \ one \ of \ the \ neihbour \ j \in {\mathcal N_i} \\
0; \ otherwise\\
\end{array}
\right.
\end{align*}
$where, \ i \in (1, 2, 3, .... , N)$
 \par The algorithm starts with one of the feasible solutions and gradually converges to an optimal or near-optimal solution, one such feasible solution would be to start with number of colors equal to the number of vertices. We aim to find the minimum number of colors to color the graph such that no vertex has a bad edge and this can be defined as the follows,
\begin{align}
& \textsc{ Graph coloring}:
\nonumber  \\
&\min_{{\bf c}\in {\bf C}_{E_i}}  F(c)  = \min_{{\bf c}\in {\bf C}_{E_i}} \mathcal K
\end{align}
$where, \ {\bf C}_{E_i} = \{ c \in C^K \mid \lvert E_i \rvert = 0 \}$


\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm with Coloring\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; and $v_i = c_k$, for all  $i\in{\mathcal L}$; $k \in (1, 2, .... m)$ \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (at time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{f(n)}$\\
4: Select a location $i$  uniformly and performs coloring operation; \\ 
5: Now select a color $c_k$ uniformly for each location $i \in c_k$; \\ 
6: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}, \  i \in C_k $  uniformly;\\
7: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i \in C_k\}$;  \\
{\bf Test phase}(in time slot n)\\ 
8: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
9:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
10: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  go back to step $3$ (selection phase);\\
11: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
12: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 13: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$)\\
\hline
\end{tabular}
\end{small}
\caption{The Pseudocode for the simulated annealing algorithm using Coloring.}\label{algo2}
\label{fig6}
\end{figure}

\textbf{Coloring Operation}: A vertex is uniformly selected and assigned with a different color, the rest of the vertices remain with previously assigned colors. If the new color doesn't conflict with other vertices in the neighborhood of the chosen vertex, then this color shall be assigned temporarily to the chosen vertex. Later this new color setting shall be tested against the previous setting. If the current setting has fewer colors compared to the previous setting, then the earlier color of the chosen vertex will be replaced by the latest color.

The algorithm shown in Fig.~\ref{algo2} is an updated version of simulated annealing algorithm mentioned earlier, this new version includes the coloring process which helps the algorithm to converge quickly. In this updated version, step $4$ runs the coloring operation then produces groups of independent locations, step $5$ selects a new color (it contains independent locations) and runs the testing and decision phase for each location that belongs to the selected color by assigning a randomly selected new threshold. This algorithm performs coloring operation and threshold validation simultaneously. 
During each iteration, threshold validation is performed on all locations that belong to a color, where as previous algorithm validates only one location per iteration. This idea of parallel validation helps the overall algorithm to converge faster. The number of colors needed to color the vertices decreases over time (i.e, number of vertices in the remaining colors will increase), which boosts the convergence speed. Thus temperature cooling for the updated algorithm is in general quicker than in the basic version. The numerical section contains specific results showcasing the relative advantage in terms of convergence time.


==> sections/shadow6.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}~\label{sec5}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 
%\begin{figure}[t!]
%\includegraphics[width=0.5\textwidth]{Pictures/flowdiagrams}
%\caption{Joint aging control and offloading}
%\end{figure}
%
\subsection{Pricing as a tool for joint aging control and offloading }

We recall that the SP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the average size of the collected data.  

First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for SP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}\label{eq:Yij}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p}) 
%\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}

\subsection{Pricing through constrained optimization}

Next, we specialize the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec4} under the  \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec3}. By using \eqref{eq:Yij}, the resulting joint problem is posed as follows: 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where we have explicited $y_{ij}$, that is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for SP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.

Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult by the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.  
%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  

\subsection{Simulated annealing for optimal pricing }

In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which $s_l=t$ means a devices upload collected data at location $l$ only if its age exceeds $t$. Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$.  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation of Joint  Offloading and Aging Control becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{ {\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$

%Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimisation problems \cite{pincus70,connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 

The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use  the probability distribution Boltzmann-Gibbs, which is  constructed for  our JOINT OFFLOADING AND AGING CONTROL by 
\begin{equation}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that 

$$\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

We now  construct the transition of the Markov chain, named $Q_T$,  that can be used to obtaining a sequence of samples from the probability distribution $\pi_T({\bf s})$.  We star by defining a symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$ as follows
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L . t_{max} }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}

The transition matrix of the Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$,  for a given temperature $T$, can be  constructed as follows : 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  {\bf s}\not={\bf s}'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  {\bf s}\not={\bf s}'\
\sum_{{\bf z}}q^*({\bf s}, {\bf z}) (1-\min\{1, \frac{\pi_T({\bf z})}{ \pi_T({\bf s})}\} ) &\textrm{ if } s_i=s_i'\\
\end{array}
\right.
\end{align}
It is shown in \cite{Hammaersly64} that a Markov chain with the above transition admits $\pi_T({\bf s})$ as stationary distribution.  

%\begin{table}
%\caption{Notation for SA algorithm}
%\begin{tabular}{ll}
%\hline
%Variable & Description \\
%\hline
%\hline
%$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
%$\mathcal{N}$ & physical  adjacency matrix \\
%$Q$ & infinitesimal generating matrix \\
%$T$ & temperature of SA algorithm \\
%$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
%${\pi}_i$ & steady state occupancy of cell $i$ \\ 
%$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
%$s$ & vector of thresholds \\
%\hline
%\end{tabular}
%\end{table}
%

The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.

\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{log(n)}$\\
4: SP selects a location $i$  uniformly; \\
5: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly;
6: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$;  \\
{\bf Test phase}(in time slot n)\\ 
7: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
8:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
9: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  comeback to step 3 (selection phase);\\
10: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
11: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 12: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Simulated annealing}


Hereafter, we present how to implement the  simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: selction, testing  and decision.  Algorithm \ref{fig4}  presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem. 

In Line 1, we initiate the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the SP selects a location uniformly. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-11,  test if the new generated state ${\bf s}(t)$ is accepted or not. Line 12  sets the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution can be done similarly to that of \cite{Bremaud99} based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

\subsection{Simulated annealing with coloring}
One of the common drawbacks of the SA algorithm mentioned in the literature is longer run time, for this reason, we propose a method to improve the run time. This can be achieved by dividing cells into independent sets such that no set contains a cell and its neighbor and test all the cells in one such set per each temperature setting as opposed to testing one cell per each temperature setting. This is achieved by transforming the cell topology as a graph with cells as vertices, connecting each cell with its neighbors with an edge, and modeling it as \textsc{Graph Coloring Problem (GCP)}, a well-studied problem in graph theory.

The aim of this problem is to fully color the graph with a minimum number of colors, which is often referred to as \textit{chromatic number}. A large part of the literature is focused on coloring the graph given a number of colors \cite{coloring1}\cite{coloring2}, which doesn't address the problem of obtaining chromatic number or near-optimal minimum colors. \cite{Kirkpatrick671}\cite{SAcoloring1}\cite{SAcoloring2} address optimization by simulated annealing and \textsc{GCP} in greater detail. Obtaining the minimum number of colors is achieved using the SA algorithm, However, it is achieved rather in an indirect way. For this reason, we propose a simple and straight forward algorithm which is very similar in its structure to the SA algorithm described in the previous section. This algorithm is illustrated in fig.\ref{fig6}. Inspiration is drawn from \cite{SAcoloring2}, however the implementation is different from it. Let us consider a set of vertices drawn from the cell topology $ {\bf v} = \lbrace v_1, v_2, v_3, . . . v_N\rbrace$, set of colors used to color vertices are ${\bf c} = \lbrace c_1 , c_2, c_3, . . . c_K \rbrace$ and 
\begin{align*}
{\mathcal E_i} =
 \left\{
\begin{array}{ll}
1; \ if \ vertex \ i \ contains \ a \ bad \ edge \ with \\ \hspace{0.4cm}atleast \ one \ of \ the \ neihbour \ j \in {\mathcal N_i} \\
0; \ otherwise\\
\end{array}
\right.
\end{align*}
$where, \ i \in (1, 2, 3, .... , N)$
 \par The algorithm starts with one of the feasible solutions and gradually converges to an optimal or near-optimal solution, one such feasible solution would be to start with number of colors equal to the number of vertices. We aim to find the minimum number of colors to color the graph such that no vertex has a bad edge and this can be defined as the follows,
\begin{align}
& \textsc{ Graph coloring}:
\nonumber  \\
&\min_{{\bf c}\in {\bf C}_{E_i}}  F(c)  = \min_{{\bf c}\in {\bf C}_{E_i}} \mathcal K
\end{align}
$where, \ {\bf C}_{E_i} = \{ c \in C^K \mid \lvert E_i \rvert = 0 \}$


\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; and $v_i = c_k$, for all  $i\in{\mathcal L}$; $k \in (1, 2, .... m)$ \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{f(n)}$\\
4: Select a location $i$  uniformly and performs coloring operation; \\ 
5: Now select a color $c_k$ uniformly \\

for each location $i \in c_k$ ; \\ 
6: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}, \  i \in C_k $  uniformly;
7: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i \in C_k\}$;  \\
{\bf Test phase}(in time slot n)\\ 
8: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
9:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
10: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  comeback to step 3 (selection phase);\\
11: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
12: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 13: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Updated Pseudocode for the simulated annealing algorithm.}\label{algo2}
\label{fig6}
\end{figure}

\textbf{Coloring Operation}: A vertex is uniformly selected and assigned with a different color, the rest of the vertices remain with previously assigned colors. If the new color doesn't conflict with other vertices in the neighborhood of the chosen vertex, then this color shall be assigned temporarily to the chosen vertex. Later this new color setting shall be tested against the previous setting. If the current setting has fewer colors compared to the previous setting, then the earlier color of the chosen vertex will be replaced by the latest color.

The algorithm shown in \ref{algo2} is an updated version of simulated annealing algorithm mentioned earlier, thsis new version includes the coloring process which helps the algorithm to converge faster. In this updated version, step $4$ runs the coloring operation then produces groups of independent locations, step $5$ selects a new color over multiple independent locations and runs the testing and decision phase for each location that belongs to the selected color by assigning a randomly selected new threshold. This algorithm performs coloring operation and threshold validation simultaneously. During each iteration, the threshold policy validation is performed on all locations which have same color. The speed up is granted by the fact that thresholds validation is performed whereas the previous algorithm validates only one location per iteration. Parallel validation lets the overall algorithm to converge faster. The number of colors needed to color the vertices decrease over time (i.e, number of vertices in the remaining colors will increase), which boosts the convergence speed. Thus temperature cooling for the updated algorithm is in general quicker than in the older version. The numerical section contains the results that showcases this difference.

==> sections/simulation.tex <==
 \begin{comment}
 \begin{figure}[t]p_3
	\centering 
	\includegraphics[width=0.5\columnwidth]{./pictures/voronoi.png}
	\caption{Voronoi tessellation for the Cologne mobility trace.} 
	\label{Voronoi}
    \end{figure}
\end{comment}
 
 \section{evaluation}\label{sec6}
 
To validate our theoretical results, we use  vehicular mobility traces of the city of Cologne (Germany), covering a region of 400 km$^2$ in a period of $24$ hours in a typical work day, involving more than $700,000$ individual vehicles. The dataset is available at \cite{cologne}. This dataset comprises the list of users' position records, each record including a sampling timestamp, the user ID, and her position in $(x,y)$ cartesian coordinates. Positions are sampled each second. User mobility is spanned across $230$ (macro) cells and the coverage of each cell is determined a posteriori according to the Voronoi tessellation  shown in Fig.~\ref{fig:price}a.  In order to generate the transition probability across cells, we have restricted to a subset of records corresponding to one hour of trace data. Then, we have resampled our dataset at $2$ second intervals to discretize the process: within such a time step the probability for a user to cross two cells is  bounded below by $0.05$.

In the first set of experiments, we have validated our aging control policy on real-world traces. The computation of the optimal policy using the proposed model requires to estimate the transitions of the Markov chain $\Gamma$, $U(x)$ and \shadow price $p_l$ of each location $l\in {\mathcal L}$. In our reference setting, the utility of message decays linearly over time, and remains zero afterwards, $U(x)=\max(M-x,0)$. We assume that the device will collect data as soon as the existing data is uploaded. Performance of the policy is evaluated over $67$ epochs corresponding to a total duration of $134$s for a device: at each epoch a device would either upload or not based on the multi-threshold  policy obtained from the model.  All $230$ locations are divided into $3$ effective groups, namely Range1, Range2, and Range3, corresponding each to a specific cost $C_1$, $C_2$, and $C_3$, respectively, sorted in  ascending order. The idea is that the location with higher cost would be configured with higher \shadow price. The results displayed in this section are configured with three prices $(p_1,p_2,p_3)$, $m_1=0$,  two effective threshold values $(m_2, m_3)$ and $M$ = 10. Location that belong to Range 1, 2 and 3 are assigned $p_1=0$, $p_2$ and  $p_3$, respectively.

\begin{figure*}[h]
\centering
\includegraphics[scale=1.3]{./pictures/voronoi.png}
\includegraphics[scale=0.3]{./pictures/M_variation_new.eps} 
\includegraphics[scale=0.3]{./pictures/p2_variation_new.eps} 
\includegraphics[scale=0.3]{./pictures/p3_variation_new.eps}
\caption{a) Voronoi tessellation for the Cologne mobility trace b) Expected average rewards for i. theoretical model, ii. simulation and iii. exhaustive search; $p_1 = 0$, $p_2 = 6$ and $p_3=9$. c) Effect of \shadow price $p_2$ on the average reward; $p_1 =0$ and $p_3 = 9$; $M=10$. d) Effect of \shadow price $p_3$ on the average reward  $p_1 =0$ and $p_2 = 6$; $M=10$. }\label{fig:price}
\end{figure*}

Since the transition matrix $\Gamma$ is derived from traces, it is interesting to compare how the optimal policy obtained by our model compares to real traces. This verification is due since mobility traces in general are neither stationary nor memoryless. Hence, in Fig. \ref{fig:price}b we compared 1) the theoretical optimal reward predicted by our model -- i.e., using the empirical transition matrix $\Gamma$, 2) the average reward obtained simulating data collection and upload using the original real traces under the optimal policy predicted by our model and, finally, 3) the optimal reward obtained using the multi-threshold policy calculated by exhaustive search on the real traces.  The match appears quite tight and also rather insensitive to the variation of $M$.  For this experiment, we have considered $p_1 = 0$, $p_2 = 6$ and $p_3=9$. 

We now explore how \shadow prices can be used to affect the freshness of information delivered by each device. To this aim, Fig.~\ref{fig:price}c and \ref{fig:price}d illustrate how the average reward -- i.e., the average AoI minus price -- changes as function of the \shadow price. Fig.~\ref{fig:price}c is achieved by fixing $p_1$ and $p_3$  and varying $p_2$ from $2$ to $8$. It shows that the average reward decreases with price $p_2$.  Indeed, as $p_2$ becomes larger, the device has more incentive to upload the collected data to locations in Range 1. It is possible that the age of collected data becomes higher -- that is upload occurs farer from the origin site -- which explains why the average reward decreases  with $p_2$. We observe the same behavior by changing the price $p_3$ and making $p_1$ and $p_2$ fixed, as depicted in Fig.~\ref{fig:price}d. In summary, if we ignore QoS constraints, the SP should indeed tend to increase the \shadow price for locations in range $2$ and range $3$: the effect is to shift all collected traffic to locations in Range 1, which are less expensive to lease. 
\begin{comment}
\begin{figure}[h]
\centering 
\includegraphics[scale=0.12]{./pictures/M_variation_new.eps}
\caption{Expected average rewards for i. theoretical model, ii. simulation and iii. exhaustive search; $p_1 = 0$, $p_2 = 6$ and $p_3=9$.} 
\label{M_variation}
\end{figure}
\begin{figure}[t]
	\centering 
	\includegraphics[scale=0.5]{./pictures/p2_variation_new.eps}
	\caption{Effect of \shadow price $p_2$ on the average reward; $M=10$. } 	
	\label{p2_variation}
\end{figure}
\begin{figure}[htpb!]
	\centering 
	\includegraphics[scale=0.6]{./pictures/p3_variation_new.eps}
	\caption{Effect of \shadow price $P_3$ on the average reward; $M=10$. }
	\label{p3_variation}
\end{figure}
\end{comment}

Fig.~\ref{fig:load}a shows the relative volume of traffic uploaded in Range 1, 2 and 3 under optimal pricing for increasing values of the AoI constraint $d$. From this simulation results we can get some useful insights on the load balancing operated by the proposed \shadow pricing scheme. The first point on the x-axis correspond to the profile of traffic obtained under uniform flat \shadow price, that is NoStrategy (NS), meaning that all IoT traffic is uploaded where it is produced. The remaining points correspond to the optimal \shadow prices for different values of $d$.  First, we observe that it is possible to shift an important  part of traffic ($13$\%-$32$\%) towards locations in Range1 (which corresponds to price $p_1=0$). A smaller part of traffic  ($1$\%-$12$\%) is instead shifted to locations in Range3. When $d$ increases, we observe more traffic is shifted since devices have more opportunity to upload collected data in locations in Range1.  

Fig.~\ref{fig:load}b shows how the \shadow price impacts the cost incurred by the SP. A larger value of $d$ for data generated at a given location means lower sensitivity to delay, which in turn increases the probability  to upload at locations in Range 1, which explains why the total cost is ultimately decreasing with the QoS constraint $d$.
\begin{figure*}[h]
\centering
\includegraphics[scale=0.24]{./pictures/Traffic_flow_d.eps}
\includegraphics[scale=0.24]{./pictures/Cost_d.eps}
\caption{Load balancing: a)  effect of \shadow pricing for various values of $d$; $\epsilon = 0.01$ b) cost incurred by the MSP for various values of $d$} \label{fig:load}
\end{figure*}
%\begin{figure*}[t]
%%\centering
%\includegraphics[scale=0.22]{./pictures/Cost_variation.jpg}
%\caption{Convergence of average cost for a given temperature scheme ($T_n = a/n^{2.5}$)}\label{temperature}
%\end{figure*}

\begin{figure*}[h]
\centering
%\includegraphics[scale=0.28]{./pictures/20_cell_comp.eps} 
\includegraphics[scale=0.28]{./pictures/20_cell_comp_zoomed.eps} 
%\includegraphics[scale=0.28]{./pictures/230_cells_comp.eps}
\includegraphics[scale=0.28]{./pictures/230_cells_comp_zoom.eps}
\caption{a) Convergence of 20 vertex graph  b) Convergence of 230 vertex graph }\label{coloring}
\end{figure*}

\begin{figure*}[h]
\centering
\includegraphics[scale=0.11]{./pictures/compd7new.eps}
\includegraphics[scale=0.11]{./pictures/compd9new.eps} 
\includegraphics[scale=0.11]{./pictures/compd12new.eps} 
%\includegraphics[scale=0.3]{./pictures/comb_n_pow_3.eps}
\caption {Comparing convergence of two algorithms for 1) $d = 7$ 2) $d = 9 $ 3) $d = 12$} \label{fig:convergence}
\end{figure*}

Results concerning location coloring are depicted in Fig.~\ref{coloring}, we considered $d = 7$, $\epsilon$ = 0.01 (factor which determines the neighbours) and used same cell topology as mentioned for earlier numerical results. Fig.~\ref{coloring} shows convergence of minimum number of colors for two different settings, first plot has $20$ vertices and next plot has $230$ vertices in the graph resulting from the cell topology. Different temperatures are considered to test the convergence of the algorithm. The results obtained with SA algorithm is compared to the branch and bound which is more conventional and can be considered as a baseline solution for coloring algorithms. As shown in Fig.~\ref{coloring}a SA algorithm performs better than branch and bound approach; in the considered cases, the former has achieved a solution with $5$ colors whereas the latter achieves $6$ colors. This trend is reversed as the number of vertices increase, which can be observed in Fig.~\ref{coloring}b since the branch-and-bound attains the minimum number of colors and SA does not. Indeed, depending on the setting, the minimum number of colors may not be attained, but for the sake of reducing the computational time, a near-optimal solution is indeed acceptable as showed in the next set of experiments. 

In Fig.~\ref{fig:convergence}, we can observe that the average cost evaluated in the SA algorithm converges to a minimum value. For the numerical results provided in \ref{fig:convergence}, we used a $20$ macro cell topology; with no loss of generality, we have normalized the traffic generation as $\frac{NF}{T} = 1$.  We consider $d= 7$, $\epsilon = 0.01$, and the maximum threshold $t_{max} = d + 3$. The temperature used to control the number of iteration was derived by trying different configurations; the basic tradeoff is to perform a number of iterations large enough for the algorithm to converge to the minimum value and yet bound them to a maximum value for the the sake of computation time. By numerical exploration,  $T_n = a/n^{2.8}$ and $a = 10^6$ would give us the best trade-off. %; we have reported a few other temperature configurations in Fig.~\ref{fig:convergence}; 
Finally, in the same figure we included the result of use of coloring of cells to run the algorithm. It can be observed that in all the experiments the proposed coloring method fasten significantly the convergence, in practice halving the convergence time with respect to the case when SA no parallelization is employed.
% More simulations are provided in the full version \cite{techrep} and in particular  the convergence of the SA algorithm.  


==> sections/system.tex <==

%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------

\section{System description}\label{sec2}	

%----------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------
\renewcommand{\thefootnote}{\fnsymbol{footnote}}
    
	\begin{figure}[t!]
	\centering 
	\includegraphics[width=0.45\textwidth]{./pictures/General.jpg}
	\caption{A geographic region covered by multiple InPs}
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
	\label{heteroGeo}
    \end{figure}
    
    \begin{figure}[t!]
	\centering 
	\includegraphics[width=0.45\textwidth]{./pictures/heterogenious.jpg}
	\caption{A heterogeneous data collection mechanism }
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
	\label{heteroData}
    \end{figure}  
  
Given the unprecedented growth in IoT \cite{IoTprojection}, data generated by IoT sensors could play massive role in smart city applications \cite{smartcity} and other aspects of human life going forward. This growth would introduce new business opportunities, data brokerage is one such opportunity which is of interest for this work. With the willingness of smartphone users or IoT device owners to sell the data under certain privacy terms \cite{IoTmarket1}, a DB can seize the opportunity to mediate between companies

 that are interested in purchasing the data and device owners. This is more promising with the idea of creating a marketplace for data \cite{IoTmarket2}\cite{IoTmarket3}\cite{IoTmarket4}\cite{IoTmarket5}, which is essential for data brokers. With this basis, we describe a heterogeneous system of interest that is shown in Figure \ref{heteroGeo}. We begin by introducing some basic terminology.  

The  {\em Service Provider (SP)} provides Internet connectivity to {\em IoT devices}.  We consider a physical region wherein a single SP acts as a data broker. We envision a scenario where the SP would collect the data from device owners or from mobile IoT devices deployed across the region as shown in Fig.~\ref{heteroData}. To that aim, the SP federates and aggregates resources  leased from various available InPs at different locations in the considered region.  Although the latter counts with a single SP, it may be covered by multiple {\em Infrastructure Providers (InPs)} (see Fig.~\ref{heteroGeo}).  

In this work the focus is on mobile IoT devices deployed by the SP, these devices would collect data for individual or organizational use. Possible use case scenarios are numerous such as smart cities, environment monitoring and healthcare monitoring. However the focus of this work is not restricted a particular use case, it is general and can be applied to any case mentioned earlier as the underlying mechanism is similar in all the use cases. We assume that the device would collect new information only up on uploading the existing data.

Each InP provides dedicated 5G slices for IoT data collection at a certain cost.  Sensed data is relayed using a fleet of mobile devices able to upload them at the need. Ultimately, mobile relays are served through resources across a pool of base stations covered by the selected InPs infrastructures. 

Here, sensed data as shown in Fig.~\ref{heteroGeo}, is heterogeneous in nature, meaning that it belongs to variety of categories such as Health, Environment, Traffic, etc. Many IoT applications are time sensitive and the the customers of the SP  may require IoT data to comply to certain QoS requirements.  As a first step  is to specify the QoS metrics for an IoT application comprehension within standardised Service Level Agreements (SLA).  Throughout the paper, we consider the latency of delivered IoT data as our reference SLA metric since low latency is one common requirement  for many use cases such as industrial automation, Intelligent transport systems  and healthcare monitoring.   The latency, in turn, is impacted by the locations from which mobile devices upload sensed data. Note that aggregated traffic may vary significantly across regional locations, e.g., due to the presence of hotspots.

The SP  negotiates and adjusts the scale of bandwidth and service functions using {\em 5G network slicing}, namely, by orchestrating  slicing functionality across heterogeneous access technologies (5G, LTE, 3G, and WI-FI), over different site types (macro, micro, and pico base stations) and over different InPs. Ultimately, the costs of leased infrastructures  depend on chosen InPs, specific access technology supported across regional sites and IoT data collection patterns; for the sake of simplicity, we shall refer to bandwidth costs only, but the whole framework may well include also costs for  local computation and/or storage \cite{3GPPPSlices}.

In order to comply with SLA agreements for IoT data collection, the SP  dynamically determines  the resources per slice required to match current demand.  In particular, larger costs are incurred in crowded and congested locations across the considered region.  Therefore, the SP designs an  {\em IoT data collection policy} by which freshness of IoT data is traded off  against costs.  The upload of non-critical data can be deferred to occur at a location incurring smaller costs. 
 
 We assume that the SP uses dynamic pricing for load balancing purposes, to incentivize  devices not to upload data from congested locations.  Such pricing is dynamically set, e.g., based on the congestion levels. Regional locations are tagged by a price for the upload of an IoT unit data. This can is shown in Figure \ref{Pricing} where IoT device is attached to a bicycle, as it moves across the regions the sensors in the device collect information and try to upload it as per the convenience, this upload mechanism is explained in detail in the following sections. For illustration purpose we have shown the participation of just two bicycles but there could be thousands of devices attached to various other vehicles with the aim of collecting data related to numerous disciplines. One of the issues in telecommunications which draws atmost attention is congestion. Given the cosmic effect of IoT, this issue is going to be more significant than ever. Through pricing, the SP can shift the IoT traffic generated by mobile IoT devices from locations where data are sensed to less crowded ones, where leased slice resources are cheaper.
   
\section{ Traffic Offloading}\label{sec:offload}	
\label{sec3}



%\subsection{Basic concepts}	

%----------------------------------------------------------------------------------------
%----------------------------------------------------------------------------------------
We shall design \shadow pricing in order to minimize the total cost incurred by the SP. We formulate a control problem accounting for the mobility pattern of devices and the delay requirements of the IoT data collection service. At each location, the SP  selects the corresponding InPs.  Let ${\L}=\{1, 2,..,L\}$
be the set of locations.  We denote by  $B_i$ the
  maximum bandwidth at location $i$, $1 \leq i \leq L$, resulting in a maximum bandwidth vector  $\bm{B}$. % be  the corresponding vector of maximum bandwidths.
%
% Vector $\bm{B}$ is one of the inputs to the cost optimization problem posed below.  
%As it will be clear in the following sections, 

Each location is tagged with a unit \shadow price, resulting in a \shadow price vector ${\bm p}=(p(i), i\in{\L})\in{\mathcal R}_{\geq 0}^L$. 
%

    \begin{figure}[t!]
	\centering 
	\includegraphics[width=0.45\textwidth]{./pictures/Pricing_new2.jpg}
	\caption{A heterogeneous region with different shadows prices }
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
	\label{Pricing}
    \end{figure}
%Let the SP fix the price for each location according to price vector ${\bf p}=(p(l), l\in{\mathcal{L}})$.  
The price vector induces a set of $K$ different prices denoted by   ${\mathcal{P}}_K$, $\mathcal{P}_K=\{P_1,..,P_K\}$, where $P_1< \ldots <P_K$. % used by the SP.  
Prices  impact  location-dependent upload policies which determine when a mobile device should upload sensed data, based on the current age of information. The age of information represents the time elapsed from sensor reading until upload. Let $\Delta_i$ be  a random variable characterizing the  age of information -- at upload time --  for data collected at location $i$.  %  for a unit of IoT data which is generated at location $i$.
 Let $C_i$ the monetary unit cost to lease bandwidth at location $i$. Let $D_i$ be the amount of data generated by devices at location $i$ during a time slot. 
Finally, the upload control is represented by variable $Y_{ij}({\bm p})$: it represents the average traffic rate for data collected at location $i$ and uploaded at location $j$.  Notation is summarized in Table~\ref{tab:notation}.
    
%{\bf sometimes we refer to prices as $P$ and sometimes as $p$ -- is there a difference? Also, sometimes we say there are $K$ prices, and sometimes we say there are $L$, one price per location? Fix that!}


\emph{Pricing control.}\label{sec:P1}	 Next, we pose the  optimization problem faced by the SP:\\
\textsc{Traffic Offloading: } 
\begin{align}
 &\underset{{\bm{p}}}{\text{minimize}}  \sum_{i\in {\Loc}} \sum_{j\in {\Loc}}  C_j \, Y_{ij}({\bm p}) \nonumber \\
& \text{subject to}\nonumber\\
&   \hskip 5mm  \sum_{j\in {\Loc}}  Y_{ji}({\bm p}) \leq B_i  ,\; \forall i \in {\Loc} \label{eq:c1}\\
&   \hskip 5mm  \sum_{j\in {\Loc}}  Y_{ij}({\bm p}) = D_i,\; \forall i \in {\Loc}\label{eq:c2}\\
&   \hskip 5mm  \mathbb{P}( \Delta_i({\bm p}) > d) \leq \epsilon_i,\; \forall i \in {\Loc}   \label{eq:c3}\\
&  \hskip 5mm  Y_{ij} \geq 0,\;  \forall i, \forall j \in {\Loc}
\end{align}
where \eqref{eq:c1} is the per location constraint on the available bandwidth for the IoT slice, \eqref{eq:c2} is a flow conservation constraint, and 
\eqref{eq:c2} provides a tunable SLA constraint on the age of information collected at specific location $i \in {\Loc}$, depending on a target latency value $ d> 0$ and on tolerance $\epsilon_i>0$. 

\begin{figure}[h]
	\centering 
	\includegraphics[width=0.45\textwidth]{./pictures/traffic_migration1.jpg}
	\caption{Without traffic offloading mechanism }
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
	\label{nomigrration}
    \end{figure}
    
    
    \begin{figure}[h]
	\centering 
	\includegraphics[width=0.45\textwidth]{./pictures/traffic_migration2.jpg}
	\caption{With traffic offloading mechanism }
	%, Coverage with multiple prices: 5G technology is an enabler for traffic offloading, and IoT devices require aging control.  In this work, we consider the joint traffic offloading and aging control problem for 5G IoT networks.  } 
	\label{trafficmigration}
    \end{figure}

Figure \ref{nomigrration} shows the scenario in which no policy is implemented, as a result upload traffic is severely high and SP may lose part of data due to outage, on top of this cost of upload would be higher as well. Where as in Figure \ref{trafficmigration} upload traffic is well distributed as it adopted the Traffic Ofloading mechanism, as a consequence there is no over burden on any particular access point.

The main challenge  to solve the \textsc{Traffic Offloading} problem is to account for the mobility pattern of devices. In fact, they collect data at some tagged location, and they upload according to the chosen policy, in order to meet QoS requirements. In practice, once a sensing device is associated to a tagged location, it will be exposed a \shadow price available for the IoT slicing service, so that the decision to upload or not can be implemented onboard of sensing devices in a fully distributed fashion. In the next sections, we shall provide a simple algorithm able to determine the optimal price vector ${\bm p}$. Before that, in the next section we shall determine the optimal upload control for an assigned price vector. 



==> shadow/shadow1.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.

%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}



In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$. Furthermore, using a static-penalty method we transform 
the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. The new formulation becomes 
\begin{align}
& \textsc{Relaxed  Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}}    L(s,\alpha)  \nonumber \\
& L(s,\alpha)=  \sum_{j\in {\mathcal L}} Y_j(s) C_j+ \alpha^1_j (Y_j(s) - B_j)^+\alpha^2_j  (F_{\Delta_j}(d) -\epsilon_i)^+  
\label{unP1}
\end{align}
where $ \alpha^k_j $  are positive real values.  As \eqref{unP1} is to be minimized with respect to ${\bf s}$, increasing the penalty of a violated constraint to a large enough value will force the corresponding to achieve the minimum of zero, and such penalties always exist if 
the  \textsc{Joint  Offloading and Aging Control} problem is feasible.  Hence, the  \textsc{Relaxed  Offloading and Aging Control} problem is equivalent to 
the  \textsc{Joint  Offloading and Aging Control} problem as long as the penalty parameter $\alpha^1_j$ and $\alpha^2_j$ are  sufficiently large for all $j\in{\mathcal L}$.  A limitation to use the static-penalty methods is that their penalty have to be find by trial and error \cite{GVK502988711}. 



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{Relaxed  Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for unconstrained combinatorial optimisation problems which can be extended to the case of constrained ones \cite{SA-constraints}. 


SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.

For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 





The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows



\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}



The SA algorithm is based on the visit of the possible system states $z=(s,\alpha)$, i.e., threshold vectors $s$ and $\alpha$. 
\begin{align}
q(z,z')= \left\{
\begin{array}{ll}
1/\left(N (t_{max}  {\alpha}_{max} - 1)\right), & \textrm{if }  \tilde{\mathcal{N}}(z,z')=1 \\
-\sum_{\tilde{z}}{q(z,\tilde{z})}, &\textrm{if } z= z' \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
where $z$ is a column vector, $z \in \mathbb{R}^?$.


We consider two versions of the algorithm. In the first,   neighboring states differ at one coordinate. In the second, neighboring states can
differ by more than one coordinate, as far as the coordinates do not \emph{conflict} with each other.  The concept of conflict is made precise in what follows,
and involves the notion of graph colorings. We refer to the corresponding neighborhood maps as $\tilde{\mathcal{N}}_0$ and $\tilde{\mathcal{N}}_1$, respectively. Then,
\begin{align}
\tilde{\mathcal{N}}_0(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' = z + 1_{j} - 1_{k} \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
and
\begin{align}
\tilde{\mathcal{N}}_1(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' \textrm{ and } z \textrm{ do not conflict } \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}




Let $q$ an irreducible Markov kernel $q$ on $S\times {\mathbb R}^{2L}$  such that $q(z,z')>0$ if and only if $q(z',z)>0$. Let define for all $T>0$ the Markov kernel $Q_T$ on $S$ such that for any $z, z' \in S\times {\mathbb R}^{2L}$, $z\not=z'$
$$
Q_T(z,z') = q(z,z') \exp(-(L(z')-L(z))^+/T)
$$
The transition corresponds to the replacement of the current solution by a neighbouring solution. Such kernel $Q_T$ induces a unique probability distribution $\pi_T$, which is typically constructed for 
the \textsc{Joint  Offloading and Aging Control} problem by
\begin{equation}
\pi_T(z) = \frac{1}{Z} \exp^{-L(z)/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum, that $\lim_{T\to \infty} \pi_T(\{z\in S\times {\mathbb R}^{2L} \mid  L(z) = \min_{s'} L(z')\})=1$ \cite{bertsimas1993}. Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(X_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: initialize:  $s_j(0)=0$, for $j=1\ldots L$ and $\alpha^k_j(0)=0$  for $j=1\ldots L$ and $k=1, 2$. \\
2:  set starting temperature $T_0= T^0$  \\
{\bf Pick phase (in time slot n)}\\ 
3. set temperature $T_n=\frac{a}{log(n)}$\\
4: The MSN selects a location $i$  with probability $\pi_i$.\\
5:  The location $i$ has  two choices :
  \begin{itemize}
  \item select a new threshold $s_i(t) \in \{0, 1,\ldots t_{max}\}\textbackslash\{s_i(t-1)\}$ u.a.r and keep $\alpha$ unchanged, or
  \item choose a new value of $\alpha_{i}(t)\in\{(\beta^1_i, \alpha^2_i)\}\cup\{(\alpha^1_i, \beta^2_i)\}$ and keep $s_i(t)$ unchanged. 
   \end{itemize}
6: Set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$ and  $\alpha^k_j(t)=\alpha^k_j(t-1)$ for all $ j\in {\mathcal L}\textbackslash\{i\}$ and $k=1,2$. \\
{\bf Train phase}\\ 
7. Each location $j$ tests the new configuration $({ s_j}(t),\alpha(t))$\\
8. Every location $j\in {\mathcal L}$ locally measure  $L_j({ s}(t),\alpha(t))$. \\
9.  Compute $\delta_j= L_j({ s}(t),\alpha(t))-L_j({ s}(t-1),\alpha(t-1))$\\
10. Each neighbour $j\in {\mathcal N}_i$ of location $i$, sends $\delta_j$ to location $i$. \\
{\bf Decision phase} \\
11. Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$\\
12. if $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state\\
{\bf otherwise }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$\\
13:  Stop SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Constrained simulated annealing}


Hereafter, we present how to implement the constrained simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: pick, training and decision.  Alg. 1 presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem using the Lagrangian function of the \textsc{Relaxed  Offloading and Aging Control} problem. 

In Line 1, we initiale the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $n$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location using the probability distribution $\pi$.  This allows to update more frequently the threshold of crowded locations. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-12,  test if the new generated state $(s(t), \alpha(t))$ is accepted or not. Line 13  set the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	


==> shadow/shadow2.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\begin{figure}[t!]
\includegraphics[width=0.5\textwidth]{flowdiagrams}
\caption{Joint aging control and offloading}
\end{figure}



\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.

%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}

In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$. 
Furthermore, using a static-penalty method we transform 
the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. The new formulation becomes 
\begin{align}
& \textsc{Relaxed  Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}}    L(s,\alpha)  \nonumber \\
& L(s,\alpha)=  \sum_{j\in {\mathcal L}} Y_j(s) C_j+ \alpha^1_j (Y_j(s) - B_j)^+\alpha^2_j  (F_{\Delta_j}(d) -\epsilon_i)^+  
\label{unP1}
\end{align}
where $ \alpha^k_j $  are positive real values.  As \eqref{unP1} is to be minimized with respect to ${\bf s}$, increasing the penalty of a violated constraint to a large enough value will force the corresponding to achieve the minimum of zero, and such penalties always exist if 
the  \textsc{Joint  Offloading and Aging Control} problem is feasible.  Hence, the  \textsc{Relaxed  Offloading and Aging Control} problem is equivalent to 
the  \textsc{Joint  Offloading and Aging Control} problem as long as the penalty parameter $\alpha^1_j$ and $\alpha^2_j$ are  sufficiently large for all $j\in{\mathcal L}$.  A limitation to use the static-penalty methods is that their penalty have to be find by trial and error \cite{GVK502988711}. 



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{Relaxed  Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for unconstrained combinatorial optimisation problems which can be extended to the case of constrained ones \cite{SA-constraints}. 


SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.

For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 





The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows



\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}



The SA algorithm is based on the visit of the possible system states $z=(s,\alpha)$, i.e., threshold vectors $s$ and $\alpha$. 
\begin{align}
q(z,z')= \left\{
\begin{array}{ll}
1/\left(N (t_{max}  {\alpha}_{max} - 1)\right), & \textrm{if }  \tilde{\mathcal{N}}(z,z')=1 \\
-\sum_{\tilde{z}}{q(z,\tilde{z})}, &\textrm{if } z= z' \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
where $z$ is a column vector, $z \in \mathbb{R}^?$.


We consider two versions of the algorithm. In the first,   neighboring states differ at one coordinate. In the second, neighboring states can
differ by more than one coordinate, as far as the coordinates do not \emph{conflict} with each other.  The concept of conflict is made precise in what follows,
and involves the notion of graph colorings. We refer to the corresponding neighborhood maps as $\tilde{\mathcal{N}}_0$ and $\tilde{\mathcal{N}}_1$, respectively. Then,
\begin{align}
\tilde{\mathcal{N}}_0(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' = z + 1_{j} - 1_{k} \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
and
\begin{align}
\tilde{\mathcal{N}}_1(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' \textrm{ and } z \textrm{ do not conflict } \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}




Let $q$ an irreducible Markov kernel $q$ on $S\times {\mathbb R}^{2L}$  such that $q(z,z')>0$ if and only if $q(z',z)>0$. Let define for all $T>0$ the Markov kernel $Q_T$ on $S$ such that for any $z, z' \in S\times {\mathbb R}^{2L}$, $z\not=z'$
$$
Q_T(z,z') = q(z,z') \exp(-(L(z')-L(z))^+/T)
$$
The transition corresponds to the replacement of the current solution by a neighbouring solution. Such kernel $Q_T$ induces a unique probability distribution $\pi_T$, which is typically constructed for 
the \textsc{Joint  Offloading and Aging Control} problem by
\begin{equation}
\pi_T(z) = \frac{1}{Z} \exp^{-L(z)/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum, that $\lim_{T\to \infty} \pi_T(\{z\in S\times {\mathbb R}^{2L} \mid  L(z) = \min_{s'} L(z')\})=1$ \cite{bertsimas1993}. Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(X_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: initialize:  $s_j(0)=0$, for $j=1\ldots L$ and $\alpha^k_j(0)=0$  for $j=1\ldots L$ and $k=1, 2$. \\
2:  set starting temperature $T_0= T^0$  \\
{\bf Pick phase (in time slot n)}\\ 
3. set temperature $T_n=\frac{a}{log(n)}$\\
4: The MSN selects a location $i$  with probability $\pi_i$.\\
5:  The location $i$ has  two choices :
  \begin{itemize}
  \item select a new threshold $s_i(t) \in \{0, 1,\ldots t_{max}\}\textbackslash\{s_i(t-1)\}$ u.a.r and keep $\alpha$ unchanged, or
  \item choose a new value of $\alpha_{i}(t)\in\{(\beta^1_i, \alpha^2_i)\}\cup\{(\alpha^1_i, \beta^2_i)\}$ and keep $s_i(t)$ unchanged. 
   \end{itemize}
6: Set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$ and  $\alpha^k_j(t)=\alpha^k_j(t-1)$ for all $ j\in {\mathcal L}\textbackslash\{i\}$ and $k=1,2$. \\
{\bf Train phase}\\ 
7. Each location $j$ tests the new configuration $({ s_j}(t),\alpha(t))$\\
8. Every location $j\in {\mathcal L}$ locally measure  $L_j({ s}(t),\alpha(t))$. \\
9.  Compute $\delta_j= L_j({ s}(t),\alpha(t))-L_j({ s}(t-1),\alpha(t-1))$\\
10. Each neighbour $j\in {\mathcal N}_i$ of location $i$, sends $\delta_j$ to location $i$. \\
{\bf Decision phase} \\
11. Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$\\
12. if $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state\\
{\bf otherwise }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$\\
13:  Stop SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Constrained simulated annealing}


Hereafter, we present how to implement the constrained simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: pick, training and decision.  Alg. 1 presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem using the Lagrangian function of the \textsc{Relaxed  Offloading and Aging Control} problem. 

In Line 1, we initiale the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $n$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location using the probability distribution $\pi$.  This allows to update more frequently the threshold of crowded locations. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-12,  test if the new generated state $(s(t), \alpha(t))$ is accepted or not. Line 13  set the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	


==> shadow/shadow3.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\begin{figure}[t!]
\includegraphics[width=0.5\textwidth]{flowdiagrams}
\caption{Joint aging control and offloading}
\end{figure}



\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.  


%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}

In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$.  Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$,   that uses threshold $t$ ({\bf put more explications}).  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation  becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{ {\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimisation problems \cite{pincus70, hajek88, connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 

The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use  the probability distribution Boltzmann-Gibbs, which is  constructed for  our JOINT OFFLOADING AND AGING CONTROL by 
\begin{equation}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that 

$$\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

We now  construct the transition of the Markov chain, named $Q_T$,  that can be used to obtaining a sequence of samples from the probability distribution $\pi_T({\bf s})$.  We star by defining a symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$ as follows
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L . t_{max} }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}

The transition matrix of the Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$,  for a given temperature $T$, can be  constructed as follows : 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  s_i\not=s_i'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  s_i\not=s_i'\\
\sum_{{\bf s}'}q^*({\bf s}, {\bf s}') (1-\min\{1, \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\} ) &\textrm{ if } s_i=s_i'\\
\end{array}
\right.
\end{align}

It is shown in \cite{Hammaersly64} that a Markov chain with the above transition admit as stationary distribution $\{\pi_T({\bf s})\} $.  


\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}


The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{log(n)}$\\
4: MSN selects a location $i$  uniformly; \\
5: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly;
6: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$;  \\
{\bf Test phase}(in time slot n)\\ 
7: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
8:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
9: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  comeback to step 3 (selection phase);\\
10: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
11: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 12: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Simulated annealing}


Hereafter, we present how to implement the  simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: selction, testing  and decision.  Algorithm \ref{fig4}  presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem. 

In Line 1, we initiate the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location uniformly. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-11,  test if the new generated state ${\bf s}(t)$ is accepted or not. Line 12  sets the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	


==> shadow/shadow4.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\begin{figure}[t!]
\includegraphics[width=0.5\textwidth]{flowdiagrams}
\caption{Joint aging control and offloading}
\end{figure}



\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.

%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}



In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$. Furthermore, using a static-penalty method we transform 
the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. The new formulation becomes 
\begin{align}
& \textsc{Relaxed  Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}}    L(s,\alpha)  \nonumber \\
& L(s,\alpha)=  \sum_{j\in {\mathcal L}} Y_j(s) C_j+ \alpha^1_j (Y_j(s) - B_j)^+\alpha^2_j  (F_{\Delta_j}(d) -\epsilon_i)^+  
\label{unP1}
\end{align}
where $ \alpha^k_j $  are positive real values.  As \eqref{unP1} is to be minimized with respect to ${\bf s}$, increasing the penalty of a violated constraint to a large enough value will force the corresponding to achieve the minimum of zero, and such penalties always exist if 
the  \textsc{Joint  Offloading and Aging Control} problem is feasible.  Hence, the  \textsc{Relaxed  Offloading and Aging Control} problem is equivalent to 
the  \textsc{Joint  Offloading and Aging Control} problem as long as the penalty parameter $\alpha^1_j$ and $\alpha^2_j$ are  sufficiently large for all $j\in{\mathcal L}$.  A limitation to use the static-penalty methods is that their penalty have to be find by trial and error \cite{GVK502988711}. 



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{Relaxed  Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for unconstrained combinatorial optimisation problems which can be extended to the case of constrained ones \cite{SA-constraints}. 


SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.

For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 





The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows



\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}



The SA algorithm is based on the visit of the possible system states $z=(s,\alpha)$, i.e., threshold vectors $s$ and $\alpha$. 
\begin{align}
q(z,z')= \left\{
\begin{array}{ll}
1/\left(N (t_{max}  {\alpha}_{max} - 1)\right), & \textrm{if }  \tilde{\mathcal{N}}(z,z')=1 \\
-\sum_{\tilde{z}}{q(z,\tilde{z})}, &\textrm{if } z= z' \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
where $z$ is a column vector, $z \in \mathbb{R}^?$.


We consider two versions of the algorithm. In the first,   neighboring states differ at one coordinate. In the second, neighboring states can
differ by more than one coordinate, as far as the coordinates do not \emph{conflict} with each other.  The concept of conflict is made precise in what follows,
and involves the notion of graph colorings. We refer to the corresponding neighborhood maps as $\tilde{\mathcal{N}}_0$ and $\tilde{\mathcal{N}}_1$, respectively. Then,
\begin{align}
\tilde{\mathcal{N}}_0(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' = z + 1_{j} - 1_{k} \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}
and
\begin{align}
\tilde{\mathcal{N}}_1(z,z')= \left\{
\begin{array}{ll}
1, & \textrm{if } z' \textrm{ and } z \textrm{ do not conflict } \\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}




Let $q$ an irreducible Markov kernel $q$ on $S\times {\mathbb R}^{2L}$  such that $q(z,z')>0$ if and only if $q(z',z)>0$. Let define for all $T>0$ the Markov kernel $Q_T$ on $S$ such that for any $z, z' \in S\times {\mathbb R}^{2L}$, $z\not=z'$
$$
Q_T(z,z') = q(z,z') \exp(-(L(z')-L(z))^+/T)
$$
The transition corresponds to the replacement of the current solution by a neighbouring solution. Such kernel $Q_T$ induces a unique probability distribution $\pi_T$, which is typically constructed for 
the \textsc{Joint  Offloading and Aging Control} problem by
\begin{equation}
\pi_T(z) = \frac{1}{Z} \exp^{-L(z)/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum, that $\lim_{T\to \infty} \pi_T(\{z\in S\times {\mathbb R}^{2L} \mid  L(z) = \min_{s'} L(z')\})=1$ \cite{bertsimas1993}. Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(X_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: initialize:  $s_j(0)=0$, for $j=1\ldots L$ and $\alpha^k_j(0)=0$  for $j=1\ldots L$ and $k=1, 2$. \\
2:  set starting temperature $T_0= T^0$  \\
{\bf Pick phase (in time slot n)}\\ 
3. set temperature $T_n=\frac{a}{log(n)}$\\
4: The MSN selects a location $i$  with probability $\pi_i$.\\
5:  The location $i$ has  two choices :
  \begin{itemize}
  \item select a new threshold $s_i(t) \in \{0, 1,\ldots t_{max}\}\textbackslash\{s_i(t-1)\}$ u.a.r and keep $\alpha$ unchanged, or
  \item choose a new value of $\alpha_{i}(t)\in\{(\beta^1_i, \alpha^2_i)\}\cup\{(\alpha^1_i, \beta^2_i)\}$ and keep $s_i(t)$ unchanged. 
   \end{itemize}
6: Set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$ and  $\alpha^k_j(t)=\alpha^k_j(t-1)$ for all $ j\in {\mathcal L}\textbackslash\{i\}$ and $k=1,2$. \\
{\bf Train phase}\\ 
7. Each location $j$ tests the new configuration $({ s_j}(t),\alpha(t))$\\
8. Every location $j\in {\mathcal L}$ locally measure  $L_j({ s}(t),\alpha(t))$. \\
9.  Compute $\delta_j= L_j({ s}(t),\alpha(t))-L_j({ s}(t-1),\alpha(t-1))$\\
10. Each neighbour $j\in {\mathcal N}_i$ of location $i$, sends $\delta_j$ to location $i$. \\
{\bf Decision phase} \\
11. Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$\\
12. if $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state\\
{\bf otherwise }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$\\
13:  Stop SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Constrained simulated annealing}


Hereafter, we present how to implement the constrained simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: pick, training and decision.  Alg. 1 presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem using the Lagrangian function of the \textsc{Relaxed  Offloading and Aging Control} problem. 

In Line 1, we initiale the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $n$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location using the probability distribution $\pi$.  This allows to update more frequently the threshold of crowded locations. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-12,  test if the new generated state $(s(t), \alpha(t))$ is accepted or not. Line 13  set the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	


==> shadow/shadow5.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\begin{figure}[t!]
\includegraphics[width=0.5\textwidth]{flowdiagrams}
\caption{Joint aging control and offloading}
\end{figure}



\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.  


%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}

In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$.  Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$,   that uses threshold $t$ ({\bf put more explications}).  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation  becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{ {\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimisation problems \cite{pincus70, hajek88, connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 

The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use  the probability distribution Boltzmann-Gibbs, which is  constructed for  our JOINT OFFLOADING AND AGING CONTROL by 
\begin{equation}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that 

$$\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

We now  construct the transition of the Markov chain, named $Q_T$,  that can be used to obtaining a sequence of samples from the probability distribution $\pi_T({\bf s})$.  We star by defining a symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$ as follows
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L . t_{max} }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}

The transition matrix of the Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$,  for a given temperature $T$, can be  constructed as follows : 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  s_i\not=s_i'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  s_i\not=s_i'\\
\sum_{{\bf s}'}q^*({\bf s}, {\bf s}') (1-\min\{1, \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\} ) &\textrm{ if } s_i=s_i'\\
\end{array}
\right.
\end{align}

It is shown in \cite{Hammaersly64} that a Markov chain with the above transition admit as stationary distribution $\{\pi_T({\bf s})\} $.  


\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}


The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{log(n)}$\\
4: MSN selects a location $i$  uniformly; \\
5: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly;
6: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$;  \\
{\bf Test phase}(in time slot n)\\ 
7: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
8:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
9: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  comeback to step 3 (selection phase);\\
10: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
11: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 12: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Simulated annealing}


Hereafter, we present how to implement the  simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: selction, testing  and decision.  Algorithm \ref{fig4}  presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem. 

In Line 1, we initiate the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location uniformly. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-11,  test if the new generated state ${\bf s}(t)$ is accepted or not. Line 12  sets the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	


==> shadow/shadow5_-_Naresh.tex <==

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

%\section{ {Aging} Aware Traffic Offloading}

\section{Joint  {Aging} Control and  Traffic Offloading}

% \section{ Optimal shadow prices}

%---------------------------------------------------------------------------------------
%--------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------------

Once we determined the optimal distributed upload control, we return to the \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. 


\begin{figure}[t!]
\includegraphics[width=0.5\textwidth]{flowdiagrams}
\caption{Joint aging control and offloading}
\end{figure}



\subsection{Pricing as a tool for joint aging control and offloading }



We recall that the MSP aims at setting optimally the value of the shadow prices in order to reduce the total cost to lease resource from different InPs. Let assume $N$ IoT devices spread over the set of locations ${\Loc}$. Each device generates data to be collected and sent to the IoT sever located in the core network every $T$ seconds. We let $\pi$ the ergodic probability that a device collects data at location $i$ is $\pi_j$ -- which in turns depends on the mobility profile of devices. Hence, the total rate of collected  data  by devices in location $j$ is given by
\begin{equation}
D_j =\frac{N \pi_j F}{T}
\end{equation}
where $F$ is the  size of collected data.  






First, observe that if shadow prices are constant over locations, i.e., $P(l)=P_1$, for $l\in {\Loc}$, each device will transmit immediately the collected data and then the total cost for MSP writes immediately
\begin{equation}
\sum_{j\in {\mathcal L}} C_j D_j=  \frac{NF}{T}\sum_{j\in {\mathcal L}}  C_j \pi_j
\end{equation}
Our primary interest for the distributed upload control via shadow pricing is to perform load balancing by shifting part of the traffic load from highly congested locations, which we expect indeed to be more expensive to lease, to lesser charged  locations. At same time, we aim at ensuring the QoS requirements of the IoT service. Under shadow pricing  vector $\bf p$, the total rate uploaded at location $j$  under the optimal threshold strategy is given by 
\begin{equation}
Y_j({\bf p}) = \sum_{i\in {\mathcal L}} Y_{ij} = \sum_{i\in {\mathcal L}} D_{i} y_{ij}({\bf p})  =  \frac{NF}{T}\sum_{i\in {\mathcal L}}  \pi_i y_{ij}({\bf p})
\label{rateu}
\end{equation}
Hence the total cost writes 
\begin{equation}
\sum_{j\in {\mathcal L}} C_j Y_j({\bf p})=  \frac{NF}{T}\sum_{j\in {\mathcal L}} C_j(\sum_{i\in {\mathcal L}} \pi_i y_{ij}({\bf p}) )
\end{equation}




\subsection{Pricing through constrained optimization}

Next, we  account for the  \textsc{Aging Control} problem introduced in Sec.~\ref{sec:problem}
 under the   \textsc{Traffic Offloading}  problem introduced in Sec.~\ref{sec:P1}. The resulting
joint problem is posed as follows. 
\begin{align}
 & \textsc{Joint  Offloading and Aging Control}: \nonumber \\
 &\hspace{10pt} \underset{{\bf p}}{\text{minimize}} \sum_{i\in {\mathcal L}}\pi_{i} \sum_{j\in {{\Loc}}}    y_{ij}({\bf p}) C_ i\\
&  \hspace{10pt} \text{subject to} \\ 
& \hspace{10pt} \hspace{10pt}  \sum_{i \in {{\Loc}}}  \pi_i y_{ij}({\bf p}) \leq f(B_j),\; \forall j \in {\mathcal L} \label{C1}\\
&  \hspace{10pt} \hspace{10pt}  \sum_{j=1}^K  y_{ij}({\bf p}) = D_i,\; \forall i \in {\mathcal L}\\
& \hspace{10pt} \hspace{10pt}  P( \Delta_i({\bf p}) > d) \leq \epsilon_i,\; \forall i \in {\mathcal L}\label{C2}\\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\end{align}
where $y_{ij}$ is the expected per device upload rate for data collected at location $i$ and uploaded at location $j$.   

We can calculate $y_{ij}({\bf p})$ based on the threshold strategy: we need to calculate the probability that a device collects data at location $i$ and uploads it at  location $j$. The calculation is performed by determining $f(i, j, t)$, namely the probability that a device collects data from location $i$ and uploads it at time $t$ in location  $j$. Such computation involves the use of taboo probability, defined as follows:
$$ 
\taboo{A\;\;}{i}{j}{\tau} = P\{l_1,..,l_{\tau-1} \not\in A, l_{\tau}=j  |  l_0=i \}, 
$$
This is the  probability   of moving from location $i$ to location $j$ in $n$ steps without entering the taboo set  $A$; such transition probabilities are calculated in the standard way by considering the $\tau$-th power of the taboo matrix, which is obtained by zeroing the columns and the rows of the transition probability matrix corresponding to the taboo states, i.e., the states in A. 
% Let define $ \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{iB}}$ be the probability  of moving from location $i$ to location in $B$ in $n$ steps without entering   taboo set   $A$. i.e.,
%$$ 
% \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{i,B}} =\sum_{j\in B}  \underset{\lbrace A\rbrace\hspace{0.4cm}}{\lambda^n_{ij}}, 
% $$
We shall define  ${{\Loc}}_i=\{l\in {{\Loc}} | p(l)\leq P_i\}$, $i=1,\ldots,K$. Based on the optimal threshold strategy, if a device collects data from a location $i\in {\mathcal L}_1$, it will immediately upload it.  Thus for  $i\in {\mathcal L}_1$, we have 
$$
f(i, z , t)= \begin{cases}
1   & \mbox{  if }   z=i \mbox{ and } t=1\\
0  & \mbox{otherwise}
\end{cases}
$$
For $i\not\in {{\Loc}}_1$ and $z\in {\mathcal L}_j$, let us consider $\widehat m_t=\max(m_j|m_j<t)$ the explicit expression can be derived as follows
\begin{comment}
\begin{eqnarray}
&&f(i, z, t)=0,  \mbox{  for }  t < t_{j}\\
&&f(i, z , t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{j+s}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {t-{t_{(j-1+s)}-1}} }}   \\
&&\hspace{2cm} \mbox{  for }  t_{j-2+s} \leq t <  t_{j-1+s},\;\; s=1..(K-j).\\
&&f(i, z, t)=\\
&&\sum_{l_1\epsilon{\mathcal L}_2^c} . .\sum_{l_{j-1+s}\epsilon{\mathcal L}_{j+s}^c} \underset{\lbrace{\mathcal L}_1\rbrace\hspace{0.5cm}}{{\lambda}_{il_1}^{\tau_1}}. . .\underset{\lbrace{\mathcal L}_{j-1+s}\rbrace\hspace{01cm}}{\lambda_{{l_{j-2+s}}{l_{j-1+s}}}^{ {\tau_{j-1+s }}}}\underset{\lbrace{\mathcal L}_{K-1}\rbrace\hspace{1.2cm}}{\lambda_{{l_{(j-1+s)-1}}z}^{ {\tau_{K-1}} }}   \\
&&\hspace{5cm} \mbox{  for }  t = t_{K-1},
\end{eqnarray}
\end{comment}
\begin{eqnarray}\label{eq:fizt}
&&\hskip-11mm f(i, z, t)=0,  \mbox{  for }  t  < m_j\\
&&\hskip-11mm f(i, z , t)=\nonumber\\
&&\hskip-11mm \sum_{l_1\not\in {\Loc}_1}\sum_{l_2\not\in {\Loc}_2} \dots \!\!\!\sum_{l_{t-1}\not\in {\Loc}_{\widehat  m_t}}  \taboo{{\Loc}_1\;}{i}{l_1}{\tau_1}\cdot \taboo{{\Loc}_2\;}{l_1}{l_2}{\tau_2}\ldots \taboo{{\Loc}_{\widehat  m_t}}{l_{t-2}}{l_{t-1}}{t-{\widehat  m_t}-1}\lambda_{l_{t-1} j}\nonumber\\
&&\hskip40mm  \mbox{  for }   m_j \leq t  \leq m_K \\
&&\hskip-11mm f(i, z, t)=0,%f(i, z, m_K),  
\mbox{  for }  m_K <  t  \leq M
%\taboo{{\Loc}_1}{i}{l_1}{\tau_1}$L_1}{i}{l_1}{\tau_1} 
\end{eqnarray}
where $\tau_k= m_{k+1} - m_{k}$, with $m_{K+1}=M$ for $k=1,\ldots,K$.  The expression of $y_{iz}$ for $z \in {{\Loc}}_j$  yields 
\begin{equation}\label{eq:yiz}
y_{iz} =\sum_{t=m_{j}}^{m_{K}} f(i,z,t)
\end{equation}
Once we obtained the values of the $f(i, z, t)$s, we can derive the stationary probability distribution for the age of information -- at the upload time -- for the data collected at location $i$, namely  $\Delta_i({\bf p})$, we obtain 
\begin{equation}\label{eq:CCDF}
F_{\Delta_i}(d):=P( \Delta_i({\bf p}) > d))= \sum_{t=d+1}^{m_{K}}  \sum_{z\in {\mathcal L}}   f(i, z, t) 
\end{equation}
Finally, the expected age of collected data from location $i\in {\mathcal L}$  is given by
\begin{equation}\label{eq:E}
 \E [ \Delta_i({\bf p})] = \sum_{t=0}^{m_{K}}  \sum_{z\in {\mathcal L}}  t \cdot f(i, z, t) 
\end{equation}
The relation \eqref{eq:CCDF} provides an important measure for MSP: it provides a metric to characterise whether an input shadow price vector can meet the requirements for the IoT data collected at a tagged location. Furthermore starting from $F_{\Delta_i}(d)$, it is possible to evaluate the deviation of the age of collected data from its average value, e.g., by using Chebishev inequality.





Solving the  \textsc{Joint  Offloading and Aging Control} problem is made difficult  the structure of function $Y$, 
which is not convex over the shadow price vectors ${\bf p}$, and, furthermore, constraints are present. 
Since the problem complexity grows rapidly in the size of the network, in what follows we propose a low complexity algorithm, which utilises 
the structure of the devices' optimal strategy to solve the problem over the set of multi-threshold policies.  


%For the sake of notation, we can denote $\C_r=\{j \in {\Loc}| C(l)=C_r\}$ the set of locations with cost $C_r$, , $r=1,\ldots,R$. Without loss of generality, we assume $C_1=0 < C_2 <\ldots <C_R$\footnote{ It sufficient to add the term $-\sum_{j\in {\mathcal{L}} }y_{ij} C_1= -C_1$ into the  objective function of $P_1$.}.  



\subsection{Pricing through relaxed optimization}

In the  \textsc{Joint  Offloading and Aging Control}  problem, the decision variable can be replaced by the threshold vector ${\bf s} =(s_1, s_2,\ldots, s_L)$ of size $L$ for which  $s_l=t$  means a devices upload its  collected data at location $t$ only if its age exceeds $t$.  Let $t_{max}$ be the maximum threshold  induced from all  pricing vectors in ${\mathbb R}^L$.  It can be calculated as follows 
$$
t_{max} = \max\{t\in {\mathbb N} \mid  P(\Delta_i (t, {\bf 0}_{-i})>d) <\epsilon_i, \forall i \in {\cal L} \}
$$
where $\Delta_j (t, {\bf 0}_{-i})$ is the delay of a collected data at location $j$ where all locations use threshold $s_i=0$ except location $j$,   that uses threshold $t$ ({\bf put more explications}).  Let define $S$ the set of threshold values, i.e., $S=\{0,1,\ldots, t_{max}\} $. 

%Furthermore, using a static-penalty method we transform 
%the  \textsc{Joint  Offloading and Aging Control} problem into an unconstrained optimisation context of SA to account for the capacity constraints as well as the QoS constraints. 
The new formulation  becomes 
\begin{align}
& \textsc{ Joint Offloading and Aging Control}: \nonumber  \\
&\min_{{\bf s}\in {\bf S}_{\epsilon,d}}  F(s,\alpha)  = \min_{{\bf s}\in {\bf S}_{\epsilon,d}}\sum_{i\in {\mathcal L}} Y_j(s) C_j\l   \\
& \hspace{10pt} \hspace{10pt} y_{ij}({\bf p}) \geq 0,\;  \forall i, \forall j \in {\mathcal L}\nonumber 
\label{unP1}
\end{align}
where ${\bf S}_{\epsilon,d} =\{ {\bf s} \in  S^{L} \mid P(\Delta_i ({\bf s})>d) <\epsilon_i,\;  Y_{i} \leq B_i, \forall i  \}$



\subsubsection{Simulated annealing}


Next, we consider simulated annealing to solve the \textsc{JOINT Offloading and Aging Control}, i.e., to minimize function~\eqref{unP1}.


Next, we introduce an efficient algorithm to solve the joint traffic offloading and aging control pricing problem.  
 The algorithm is driven by the rationale according to which a shadow price vector
  should permit to offload as much traffic as possible towards locations with smaller costs. 
In order to obtain the optimal pricing, we use the simulated annealing technique (SA), a standard technique for constrained combinatorial optimisation problems \cite{pincus70, hajek88, connnors88}. 

SA starts from a feasible solution and attempts to improve it by performing random perturbations. The procedure starts from the generation of a trial state at random and evaluates its performance objective. If the new state improves the objective function, the system jumps to this new state. If the objective of the trial state is not better off than that the current one, the trial is accepted or rejected based on a certain probabilistic criterion. The main feature of the procedure is that a worse off solution may be accepted as a new solution with a certain probability. The advantage of SA is the ability to avoid becoming trapped at local minima; furthermore, it is simple to implement in a distributed way.
%
%For a given price vector $(p_i)_{i\in {\mathcal L}}$ assigned to the $L$ locations there exists a unique optimal multi-threshold policy for devices to upload collected data. In fact, threshold $m_j$ indicates the minimum AoI needed to upload data to a location having price $P_j$: we can operate our optimal shadow price determination directly in the space of thresholds. 
%%Hence, in order to speed-up the convergence of the SA, we use the threshold vector instead shadow price vector to minimise the cost function of ${\bf P1}$. 

The neighbour structure is essential in design of  SA for our  context. Specifically, let define neighbour set ${\mathcal N}_i$ for each location $i$: location $j$  belongs to ${\mathcal N}_i$ if $j$ is located within a given radius such that data offloaded to $j$ can be impacted by traffic generated at location $i$. This means that $Y_{ij} ({\bf s}) >0 $ or $Y_{ji} ({\bf s}) >0 $ is positive for at least one threshold vector. Hence, if the location is chosen at time slot $t$, it need only to collect information from its neighbouring location $j\in{\mathcal L}$.
%For penalty parameters, we define the neighbour  of $\alpha_i=(\alpha_i^1,\alpha^2_i)$ as follows

We use  the probability distribution Boltzmann-Gibbs, which is  constructed for  our JOINT OFFLOADING AND AGING CONTROL by 
\begin{equation}
\pi_T({\bf s}) = \frac{1}{Z} \exp^{-L({\bf s})/T},
\end{equation}
where $Z$ is normalised constant. The parameter $T$ is interpreted as a temperature and, under  certain assumptions, it ensures ergodic convergence to the optimum \cite{bertsimas1993}, that 

$$\lim_{T\to \infty} \pi_T(\{{\bf s}\in S_{\epsilon, d}  \mid  L(z) = \min_{{\bf s}'} L({\bf s}')\})=1
$$ 
Overall, this method is known as the Metropolis--Hastings (MH) algorithm. 

We now  construct the transition of the Markov chain, named $Q_T$,  that can be used to obtaining a sequence of samples from the probability distribution $\pi_T({\bf s})$.  We star by defining a symmetric transition probability $Q^*=q({\bf s}, {\bf s}')$ as follows
\begin{align}
q^*({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{1}{L . t_{max} }, & \textrm{if for some }  i\in N_i, s_i\not=s_i'\\
  & \textrm{ and } s_j=s_j', \forall j\in N_i\textbackslash\{i\}\\
0, & \textrm{otherwise} \\
\end{array}
\right.
\end{align}

The transition matrix of the Markov chain, named $Q_T=(q_T({\bf s}, {\bf s}')$ $0\leq s_i,s_i'\leq t_{max}$,  for a given temperature $T$, can be  constructed as follows : 
\begin{align}
q_T({\bf s}, {\bf s}')= \left\{
\begin{array}{ll}
\frac{q^*({\bf s}, {\bf s}')  \pi_T({\bf s}')}{ \pi_T({\bf s}) } & \hspace{-2cm}\textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}<1 \textrm{ and }  s_i\not=s_i'\\
q^*({\bf s}, {\bf s}')  & \hspace{-2cm} \textrm{ if }  \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\geq 1 \textrm{ and }  s_i\not=s_i'\\
\sum_{{\bf s}'}q^*({\bf s}, {\bf s}') (1-\min\{1, \frac{\pi_T({\bf s}')}{ \pi_T({\bf s})}\} ) &\textrm{ if } s_i=s_i'\\
\end{array}
\right.
\end{align}

It is shown in \cite{Hammaersly64} that a Markov chain with the above transition admit as stationary distribution $\{\pi_T({\bf s})\} $.  


\begin{table}
\caption{Notation for SA algorithm}
\begin{tabular}{ll}
\hline
Variable & Description \\
\hline
\hline
$\tilde{\mathcal{N}}$ & adjacency  matrix of MC states \\
$\mathcal{N}$ & physical  adjacency matrix \\
$Q$ & infinitesimal generating matrix \\
$T$ & temperature of SA algorithm \\
$\tilde{\pi}(z)$ & steady state probability of state $z$ under SA algorithm  \\ 
${\pi}_i$ & steady state occupancy of cell $i$ \\ 
$\alpha$ & vector of reachable and feasible Lagrange multipliers \\
$s$ & vector of thresholds \\
\hline
\end{tabular}
\end{table}


The most distinct feature of SA is that allows $T_n$ to decrease in time, in order to guarantee the convergence to the optimal pricing.  For a temperature  $T_n$, we define an inhomogeneous Markov chain $(Y_n)_{n\in {\mathcal N}} $ with transition kernel $Q_{T_n}$ at time $n$. With a dynamics of $T_n$ sufficiently slow, the Markov chain $Q_{T_n}$ can reach a sufficiently small neighbourhood of the equilibrium  $\pi_{{T_n}}$. For this reason $T_n$ is called the cooling schedule of SA. In this paper we use the most popular cooling schedules, which are of the form  $T_n=\frac{a}{log(n)}$ where $a>0$ is a constant that determines the cooling rate order.
\begin{figure}[t]
\begin{small}
\begin{tabular}{|p{0.95\columnwidth}|}
\hline
Simulated annealing (SA) algorithm\\
\hline
%Receives: $\pi=(\pi_1,\ldots,pi_L)$\\  
%%Receives: $\blambda$, $\bmu$, and $\bd$ \\  
1: Initialize:  $s_j(0)=0$, for all  $j\in{\bf L}$; \\
2: Set starting temperature $T_0= T^0$;  \\
{\bf Selection  phase (in time slot n)}\\ 
3. Set temperature $T_n=\frac{a}{log(n)}$\\
4: MSN selects a location $i$  uniformly; \\
5: Select a  select a new threshold $s_i(t) \in  S\textbackslash\{s_i(t-1)\}$ uniformly;
6: set  $s_{j}(t)=s_{j}(t-1)$,  $\forall j\in {\mathcal L}\textbackslash\{i\}$;  \\
{\bf Test phase}(in time slot n)\\ 
7: Each location  $j\in {\mathcal L}$ locally measures $\delta_j=(Y_j({ \bf s}(t))-Y_j({ \bf s}(t-1))C_j$ and $P(\Delta_j({ \bf s}(t)>d)$; \\
8:  Each  location  $j\in {\mathcal L}$ send its measures to location $i$\\
{\bf Decision phase} \\
9: {\bf If }the new state ${\bf s}(t)$   satisfies  all constraints for all locations in $N_i$, go to step 10,\\
\hspace{0.4cm}{\bf else }  comeback to step 3 (selection phase);\\
10: Set  $\delta = \sum_{j\in N_i \cup \{i\}} \delta_{j}$;\\
11: {\bf  If} $\delta < 0$ then $(s(t-1),\alpha(t-1)$ is replaced by new state,\\
\hspace{0.4cm}{\bf else }   $(s(t),\alpha(t))=(s(t-1),\alpha(t-1))$ with probability  $1-e^{\delta/T_n}$;\\
 {\bf Stop conditions}\\ 
 12: SA when the current configuration is not changed  for a couple of successive temperatures or the current temperature $T_n$  is small enough (e.g. $T_n <10^{-6}$\\
\hline
\end{tabular}
\end{small}
\caption{Pseudocode for the simulated annealing algorithm.}\label{algo}
\label{fig4}
\end{figure}



\subsubsection{Simulated annealing}


Hereafter, we present how to implement the  simulated algorithm for solving the  \textsc{Joint  Offloading and Aging Control}  problem.  We consider  time  divided into discrete slots where each time slot $t$ consists of three phases: selction, testing  and decision.  Algorithm \ref{fig4}  presents our global minimization algorithm called SA for solving   the 
\textsc{Joint  Offloading and Aging Control} problem. 

In Line 1, we initiate the threshold for all location to zero. This corresponds that all allocation use price $p=0$.  Line 2 initialises the temperature  to be large enough to allow almost trial points to be accepted uniformly at random. At each time slot $t$, we set the temperature $T_n=\frac{a}{log(n)}$.   In line 4, the MSN selects a location uniformly. Line 5 describes how a new state is generated from selected location.  Line 6 indicates that the strategies of other location are  not changed.  Lines 7-11,  test if the new generated state ${\bf s}(t)$ is accepted or not. Line 12  sets the condition to stop the SA algorithm. 

%First we start to define the neighbourhood of state $(s,\alpha)$ in the mixed space $[0,t_{max}]^{L}\times '\mathbb{R}^+)^{2L}$.   We define a neighbour set $N_{(s,\alpha)}$  for each state as follows \cite{} :
%$$
%N_{(s,\alpha)} = \{ (s',\alpha) \mid s\in N_s \} \cup  = \{ (s,\alpha') \mid \alpha'\in N_\alpha \} 
%$$
%where $ N_\alpha = \{(\beta \mid \beta > \alpha,\; \beta^1_i=\alpha^1_i \mbox{ if }  Y_i(s)=B_i  \mbox{ and } \beta^2_i=\alpha^2_i \mbox{ if } F_{\Delta_i}(d) =\epsilon_i\}$. 
A proof of asymptotic convergence of Algorithm 1  to the optimal solution   can be done similarly to that of \cite{Bremaud99}
based on the notion of weak ergodicity of Markov chains and is thus omitted here. 
\begin{theorem}
The Markov chain modeling SA converges to the constrained optimal threshold $s^*in S^*$ with probability one, where $S^*$ is the set of the optimal solutions of the
\textsc{Joint  Offloading and Aging Control} problem.
\end{theorem}

	

